PHANGS-JWST First Results: Massive Young Star Clusters and New Insights from JWST Observations of NGC 1365

A primary new capability of JWST is the ability to penetrate the dust in star forming galaxies to identify and study the properties of young star clusters that remain embedded in dust and gas. In this paper we combine new infrared images taken with JWST with our optical HST images of the star-bursting barred (Seyfert2) spiral galaxy NGC 1365. We find that this galaxy has the richest population of massive young clusters of any known galaxy within 30 Mpc, with $\sim$ 30 star clusters that are more massive than 10$^6$ Msolar and younger than 10 Myr. Sixteen of these clusters are newly discovered from our JWST observations. An examination of the optical images reveals that 4 of 30 ($\sim$13$\%$) are so deeply embedded that they cannot be seen in the I band (AV $\gt$ 10 mag), and that 11 of 30 ($\sim$37$\%$) are missing in the HST B band, so age and mass estimates from optical measurements alone are challenging. These numbers suggest that massive clusters in NGC 1365 remain obscured in the visible for $\sim$ 1.3 $\pm$ 0.7 Myr, and are either completely or partially obscured for $\sim$ 3.7 $\pm$ 1.1 Myr. We also use the JWST observations to gain new insights into the triggering of star cluster formation by the collision of gas and dust streamers with gas and dust in the bar. The JWST images reveal previously unknown structures (e.g., bridges and overshoot regions from stars that form in the bar) that help us better understand the orbital dynamics of barred galaxies and associated star-forming rings. Finally, we note that the excellent spatial resolution of the NIRCAM F200W filter provides a better way to separate barely resolved compact clusters from individual stars based on their sizes.

==> tables/apcorr_prop_table.tex <==
\begin{table*}
\centering
\centerline{Aperture Correction Scatter}
\begin{tabular}{|c|c|c|c|c|c|}
\hline
  \multicolumn{1}{|c|}{Galaxy ID} &
  \multicolumn{1}{c|}{Avg. Ap. Corr} &
  \multicolumn{1}{c|}{Mean Ind. Corr.} &
  \multicolumn{1}{c|}{Median Ind. Corr.} &
  \multicolumn{1}{c|}{Ind. Corr. St. Dev.} &
  \multicolumn{1}{c|}{Range (max - min)} \\ 
\hline
  NGC 4826 & -0.72 & -0.64 & -0.62 & 0.26 & 1.26\\
  NGC 3351 & -0.68 & -0.57 & -0.55 & 0.26 & 1.0\\
  NGC 3627 & -0.81 & -0.67 & -0.63 & 0.21 & 0.91\\
  NGC 2835 & -0.81 & -0.67 & -0.61 & 0.28 & 1.02\\
  NGC 5248 & -0.65 & -0.56 & -0.55 & 0.19 & 0.74\\
  NGC 4571 & -0.61 & -0.52 & -0.49 & 0.19 & 0.71\\
  NGC 4689 & -0.63 & -0.53 & -0.56 & 0.14 & 0.53\\
  NGC 4569 & -0.76 & -0.66 & -0.66 & 0.22 & 0.88\\
  NGC 4535 & -0.71 & -0.58 & -0.57 & 0.15 & 0.67\\
  NGC 1792 & -0.8 & -0.65 & -0.69 & 0.18 & 0.62\\
  NGC 4548 & -0.64 & -0.53 & -0.5 & 0.28 & 1.01\\
  NGC 1566 & -0.62 & -0.55 & -0.51 & 0.2 & 0.84\\
  NGC 1433 & -0.62 & -0.54 & -0.5 & 0.23 & 0.8\\
  NGC 1559 & -0.67 & -0.57 & -0.56 & 0.18 & 0.67\\
  NGC 1365 & -0.61 & -0.52 & -0.49 & 0.24 & 1.16\\
  NGC 4654 & -0.83 & -0.64 & -0.63 & 0.18 & 0.73\\
  NGC 2775 & -0.45 & -0.45 & -0.41 & 0.21 & 0.79\\
\hline\end{tabular}
\caption{\label{tab:ap_corr_prop} This table provides further details on the aperture correction results presented in Table \ref{tab:apcor_components}. The first and second columns are repeated from Table \ref{tab:apcor_components} and show the galaxy ID, and average aperture correction, respectively. The third and fourth columns are the mean and the median of the distribution of individual cluster contributions to the aperture correction. The fifth column is the standard deviation of the same distribution. Finally, the sixth column is the minimum value of this distribution, subtracted from the maximum.}
\end{table*}

==> tables/apcorr_steps_table.tex <==
\begin{table*}
\centering
\centerline{Aperture Corrections of PHANGS-HST Galaxies}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
\hline
  \multicolumn{1}{|c|}{Galaxy ID} &
  \multicolumn{1}{c|}{$d \pm \delta d$} &
  \multicolumn{1}{c|}{Avg. Ap. Corr.} &
  \multicolumn{1}{c|}{Step 1 Cont.}  &
  \multicolumn{1}{c|}{Step 2 Cont.} &
  \multicolumn{1}{c|}{Step 3 Cont.} &
  \multicolumn{1}{c|}{Total Cat. 1} &
  \multicolumn{1}{c|}{Viable Cat. 1} &
  \multicolumn{1}{c|}{Total Cat. 2} &
  \multicolumn{1}{c|}{Viable Cat. 2} \\
\hline
  NGC 4826 & ~4.41$\pm$0.19 & -0.72 & -0.573 & -0.127 & -0.023 & 11 & 10 & 10 & 10\\
  NGC 3351 & ~9.96$\pm$0.33 & -0.68 & -0.532 & -0.134 & -0.018 & 12 & 10 & 11 & 10\\
  NGC 3627 & 11.32$\pm$0.48 & -0.81 & -0.613 & -0.191 & -0.004 & 10 & 10 & 9 & 9\\
  NGC 2835 & 12.22$\pm$0.94 & -0.81 & -0.618 & -0.178 & -0.019 & 10 & 9 & 11 & 11\\
  NGC 5248 & 14.87$\pm$1.34 & -0.65 & -0.488 & -0.157 & -0.009 & 10 & 9 & 9 & 9\\
  NGC 4571 & 14.9~$\pm$1.1 & -0.61 & -0.416 & -0.172 & -0.017 & 10 & 9 & 10 & 8\\
  NGC 4689 & 15.00~$\pm$2.25 & -0.63 & -0.497 & -0.12 & -0.018 & 10 & 9 & 10 & 10\\
  NGC 4569 & 15.76$\pm$2.36 & -0.76 & -0.541 & -0.212 & -0.004 & 10 & 10 & 10 & 9\\
  NGC 4535 & 15.77$\pm$0.37 & -0.71 & -0.533 & -0.166 & -0.013 & 12 & 10 & 10 & 8\\
  NGC 1792 & 16.20~$\pm$2.43 & -0.8 & -0.614 & -0.185 & -0.005 & 10 & 9 & 10 & 10\\
  NGC 4548 & 16.22$\pm$0.38 & -0.64 & -0.456 & -0.162 & -0.025 & 11 & 11 & 9 & 8\\
  NGC 1566 & 17.69$\pm$2.00 & -0.62 & -0.496 & -0.114 & -0.015 & 16 & 16 & 10 & 10\\
  NGC 1433 & 18.63$\pm$1.86 & -0.62 & -0.51 & -0.096 & -0.019 & 11 & 8 & 10 & 10\\
  NGC 1559 & 19.44$\pm$0.45 & -0.67 & -0.52 & -0.138 & -0.011 & 18 & 17 & 8 & 7\\
  NGC 1365 & 19.57$\pm$0.78 & -0.61 & -0.505 & -0.099 & -0.009 & 16 & 14 & 10 & 10\\
  NGC 4654 & 21.98$\pm$1.16 & -0.83 & -0.576 & -0.247 & -0.007 & 10 & 8 & 10 & 8\\
  NGC 2775 & 23.15$\pm$3.47 & -0.45 & -0.371 & -0.071 & -0.01 & 12 & 10 & 7 & 5\\
\hline\end{tabular}
\caption{\label{tab:apcor_components} Table showing the final aperture corrections per galaxy, contributions from individual steps detailed in Section~\ref{sec:ap_corr}, and numbers of clusters from the bright, isolated sample used for the measurement. The first column is the galaxy ID. Second column shows the distance to the galaxy with its uncertainty, as compiled by \citet{Anand21}. Third column shows the final average aperture correction derived for the galaxy. Columns through four to six display the contributions from the steps detailed in Section~\ref{sec:ap_corr}. Columns~7 and~8 show the total number of class~1 objects in the sample, and those that satisfy the viability conditions of Section~\ref{subsec:quality_cuts}, respectively. Columns~9 and~10 display the same quantities but for category 2 clusters.}  %(SD: Significant figures to be corrected)}
\end{table*}

==> tables/photometry_table.tex <==

\begin{sidewaystable}
\small
%\begin{table*}
\centering
\begin{tabularx}{\textwidth}{@{} *{25}{C} @{} }
\toprule
Object ID & Galaxy & RA & Dec & X & Y & F275W\_VEGA & F275W\_VEGA\_ERR & F336W\_VEGA & F336W\_VEGA\_ERR & F438W\_VEGA & F438W\_VEGA\_ERR & F555W\_VEGA & F555W\_VEGA\_ERR & F814W\_VEGA & F814W\_VEGA\_ERR & Age & Age_err & Mass & Mass_err & EBV & EBV_err & M20 & Class \\ 
\midrule
  53.381819\_-36.137701 & ngc1365 & 53.38182 & -36.1377 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & -1.71 & 1.0\\
  53.400308\_-36.11964 & ngc1365 & 53.40031 & -36.11964 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & -1.69 & 1.0\\
  53.398447\_-36.135902 & ngc1365 & 53.39845 & -36.1359 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & -1.64 & 1.0\\
  53.40409\_-36.130023 & ngc1365 & 53.40409 & -36.13002 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & -1.63 & 1.0\\
  53.417391\_-36.124742 & ngc1365 & 53.41739 & -36.12474 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & -1.72 & 1.0\\
  53.39593\_-36.139797 & ngc1365 & 53.39593 & -36.1398 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & -1.76 & 1.0\\
  53.417868\_-36.166208 & ngc1365 & 53.41787 & -36.16621 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & -1.62 & 1.0\\
  53.41594\_-36.14268 & ngc1365 & 53.41594 & -36.14268 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & -1.87 & 1.0\\
  53.399613\_-36.146323 & ngc1365 & 53.39961 & -36.14632 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & -1.59 & 1.0\\
  53.406428\_-36.141698 & ngc1365 & 53.40643 & -36.1417 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & -1.59 & 1.0\\
  53.430323\_-36.132121 & ngc1365 & 53.43032 & -36.13212 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & -1.52 & 2.0\\
  53.43111\_-36.147136 & ngc1365 & 53.43111 & -36.14714 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & -1.68 & 2.0\\
  53.401377\_-36.12849 & ngc1365 & 53.40138 & -36.12849 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & -1.57 & 2.0\\
  53.435189\_-36.139933 & ngc1365 & 53.43519 & -36.13993 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & -1.38 & 2.0\\
  53.399865\_-36.141831 & ngc1365 & 53.39987 & -36.14183 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & -1.6 & 2.0\\
  53.399546\_-36.141117 & ngc1365 & 53.39955 & -36.14112 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & -1.7 & 2.0\\
  53.407326\_-36.135808 & ngc1365 & 53.40733 & -36.13581 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & -1.55 & 2.0\\
  53.43025\_-36.135722 & ngc1365 & 53.43025 & -36.13572 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & -1.63 & 2.0\\
  53.428914\_-36.134957 & ngc1365 & 53.42891 & -36.13496 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & -1.78 & 2.0\\
  53.428664\_-36.13551 & ngc1365 & 53.42866 & -36.13551 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & -1.6 & 2.0\\
  53.428044\_-36.130439 & ngc1365 & 53.42804 & -36.13044 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & -1.35 & 3.0\\
  53.428552\_-36.131517 & ngc1365 & 53.42855 & -36.13152 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & -1.02 & 3.0\\
  53.429242\_-36.137642 & ngc1365 & 53.42924 & -36.13764 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & -0.77 & 3.0\\
  53.429187\_-36.138038 & ngc1365 & 53.42919 & -36.13804 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & -1.19 & 3.0\\
  53.407887\_-36.1353 & ngc1365 & 53.40789 & -36.1353 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & -0.96 & 3.0\\
  53.381924\_-36.148614 & ngc1365 & 53.38192 & -36.14861 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & -0.8 & 3.0\\
  53.372536\_-36.152668 & ngc1365 & 53.37254 & -36.15267 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & -1.11 & 3.0\\
  53.380433\_-36.155856 & ngc1365 & 53.38043 & -36.15586 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & -0.89 & 3.0\\
  53.389071\_-36.154691 & ngc1365 & 53.38907 & -36.15469 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & -0.78 & 3.0\\
  53.419558\_-36.168288 & ngc1365 & 53.41956 & -36.16829 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & -0.7 & 3.0\\
  53.396977\_-36.140089 & ngc1365 & 53.39698 & -36.14009 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & -1.79 & 1.0\\
  53.397563\_-36.139837 & ngc1365 & 53.39756 & -36.13984 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & -1.76 & 1.0\\
  53.397628\_-36.139071 & ngc1365 & 53.39763 & -36.13907 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & -1.77 & 1.0\\
  53.403672\_-36.135748 & ngc1365 & 53.40367 & -36.13575 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & -1.87 & 1.0\\
  53.415059\_-36.133952 & ngc1365 & 53.41506 & -36.13395 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & -1.73 & 1.0\\
  53.418855\_-36.128265 & ngc1365 & 53.41886 & -36.12826 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & -1.44 & 1.0\\
  55.518851\_-47.224922 & ngc1433 & 55.51885 & -47.22492 & 4631.26 & 4690.39 & 23.41 & 0.16 & 22.76 & 0.08 & 22.97 & 0.03 & 22.38 & 0.01 & 21.27 & 0.02 & 5.0 & 66.0 & 10012.67 & 16894.06 & 0.9 & 0.39 & -1.79 & 1.0\\
  55.51648\_-47.21752 & ngc1433 & 55.51648 & -47.21752 & 4777.61 & 5362.91 & 23.24 & 0.13 & 22.53 & 0.06 & 22.62 & 0.02 & 21.99 & 0.01 & 20.87 & 0.01 & 118.0 & 92.0 & 54686.56 & 4341.54 & 0.53 & 0.09 & -1.75 & 1.0\\
  55.52586\_-47.213615 & ngc1433 & 55.52586 & -47.21362 & 4198.65 & 5717.67 & 22.5 & 0.08 & 21.85 & 0.04 & 21.93 & 0.01 & 21.38 & 0.01 & 20.26 & 0.01 & 136.0 & 60.0 & 87612.56 & 144.83 & 0.47 & 0.08 & -1.6 & 1.0\\
  55.529474\_-47.221714 & ngc1433 & 55.52947 & -47.22171 & 3975.72 & 4981.74 & 22.59 & 0.08 & 22.08 & 0.05 & 22.1 & 0.02 & 21.54 & 0.01 & 20.41 & 0.01 & 136.0 & 41.0 & 75450.27 & 2202.51 & 0.47 & 0.08 & -1.78 & 1.0\\
  55.509882\_-47.215447 & ngc1433 & 55.50988 & -47.21545 & 5184.8 & 5551.28 & 23.01 & 0.11 & 22.57 & 0.07 & 22.55 & 0.02 & 21.89 & 0.01 & 20.7 & 0.01 & 110.0 & 8.0 & 63165.01 & 10800.4 & 0.56 & 0.04 & -1.61 & 1.0\\
  55.477804\_-47.221491 & ngc1433 & 55.4778 & -47.22149 & 7164.34 & 5001.67 & 24.85 & 0.54 & 23.03 & 0.09 & 22.76 & 0.03 & 21.92 & 0.01 & 20.5 & 0.01 & 2440.0 & 1550.0 & 190228.43 & 52923.37 & 0.15 & 0.21 & -1.88 & 1.0\\
  55.50394\_-47.239948 & ngc1433 & 55.50394 & -47.23995 & 5551.27 & 3324.97 & 22.54 & 0.07 & 22.76 & 0.08 & 23.1 & 0.03 & 22.95 & 0.02 & 22.26 & 0.02 & 95.0 & 29.0 & 6114.07 & 978.02 & 0.12 & 0.02 & -1.48 & 1.0\\
  55.498284\_-47.203477 & ngc1433 & 55.49828 & -47.20348 & 5901.06 & 6639.0 & 23.9 & 0.22 & 23.77 & 0.17 & 24.01 & 0.07 & 23.81 & 0.03 & 23.35 & 0.06 & 226.0 & 79.0 & 2945.13 & 565.9 & 0.0 & 0.02 & -1.57 & 1.0\\
  55.51437\_-47.202646 & ngc1433 & 55.51437 & -47.20265 & 4907.67 & 6714.36 & 24.38 & 0.37 & 23.78 & 0.18 & 24.08 & 0.08 & 23.46 & 0.02 & 22.19 & 0.02 & 6.0 & 65.0 & 3026.58 & 7008.0 & 0.82 & 0.33 & -1.56 & 1.0\\
  55.531585\_-47.236019 & ngc1433 & 55.53158 & -47.23602 & 3845.75 & 3681.9 &  & -0.67 & 26.57 & 2.16 & 24.61 & 0.12 & 23.73 & 0.03 & 22.38 & 0.03 & 717.0 & 559.0 & 26859.38 & 9008.42 & 0.45 & 0.2 & -1.56 & 1.0\\
  55.489504\_-47.228408 & ngc1433 & 55.4895 & -47.22841 & 6441.7 & 4373.09 & 24.07 & 0.28 & 23.61 & 0.17 & 23.79 & 0.06 & 23.15 & 0.02 & 22.05 & 0.02 & 5.0 & 191.0 & 4874.99 & 13990.8 & 0.9 & 0.47 & -1.67 & 1.0\\
  55.505925\_-47.244901 & ngc1433 & 55.50592 & -47.2449 & 5428.45 & 2875.04 & 21.65 & 0.03 & 21.83 & 0.04 & 23.11 & 0.03 & 23.01 & 0.02 & 22.64 & 0.03 & 1.0 & 0.0 & 3414.75 & 542.99 & 0.41 & 0.04 & -1.6 & 2.0\\
  55.536929\_-47.212441 & ngc1433 & 55.53693 & -47.21244 & 3515.49 & 5824.24 & 19.96 & 0.01 & 20.31 & 0.02 & 21.62 & 0.02 & 21.63 & 0.01 & 21.41 & 0.02 & 1.0 & 0.0 & 9277.64 & 1105.81 & 0.32 & 0.03 & -1.84 & 2.0\\
  55.539137\_-47.212626 & ngc1433 & 55.53914 & -47.21263 & 3379.12 & 5807.38 & 20.16 & 0.02 & 20.68 & 0.02 & 22.26 & 0.02 & 22.42 & 0.02 & 22.48 & 0.04 & 1.0 & 0.0 & 2330.07 & 270.02 & 0.11 & 0.03 & -1.59 & 2.0\\
  55.513315\_-47.205829 & ngc1433 & 55.51332 & -47.20583 & 4972.87 & 6425.4 & 18.55 & 0.01 & 19.15 & 0.01 & 20.65 & 0.01 & 20.78 & 0.01 & 20.77 & 0.02 & 1.0 & 2.0 & 11623.27 & 3329.66 & 0.14 & 0.01 & -1.29 & 2.0\\
  55.511978\_-47.20022 & ngc1433 & 55.51198 & -47.20022 & 5055.75 & 6935.33 & 20.16 & 0.02 & 20.46 & 0.02 & 22.03 & 0.02 & 21.76 & 0.01 & 21.36 & 0.02 & 8.0 & 0.0 & 1707.56 & 205.73 & 0.01 & 0.03 & -1.58 & 2.0\\
  55.496546\_-47.239217 & ngc1433 & 55.49655 & -47.23922 & 6007.6 & 3391.04 & 21.0 & 0.02 & 21.35 & 0.03 & 22.79 & 0.03 & 22.71 & 0.02 & 22.29 & 0.03 & 8.0 & 0.0 & 741.55 & 57.91 & 0.0 & 0.02 & -1.52 & 2.0\\
  55.537997\_-47.230764 & ngc1433 & 55.538 & -47.23076 & 3450.14 & 4159.1 & 20.83 & 0.02 & 21.4 & 0.03 & 22.98 & 0.04 & 23.09 & 0.02 & 23.09 & 0.06 & 1.0 & 0.0 & 1286.48 & 224.85 & 0.12 & 0.04 & -1.77 & 2.0\\
  55.541537\_-47.230541 & ngc1433 & 55.54154 & -47.23054 & 3231.13 & 4179.52 & 19.48 & 0.01 & 20.08 & 0.01 & 21.63 & 0.01 & 21.75 & 0.01 & 21.72 & 0.02 & 1.0 & 0.0 & 4654.38 & 529.14 & 0.13 & 0.03 & -1.68 & 2.0\\
  55.522164\_-47.238589 & ngc1433 & 55.52216 & -47.23859 & 4427.04 & 3448.58 & 19.52 & 0.01 & 19.8 & 0.01 & 21.07 & 0.01 & 21.02 & 0.01 & 20.68 & 0.01 & 1.0 & 0.0 & 19736.11 & 2364.26 & 0.38 & 0.03 & -1.74 & 2.0\\
  55.49227\_-47.204737 & ngc1433 & 55.49227 & -47.20474 & 6271.73 & 6523.69 & 21.68 & 0.04 & 21.88 & 0.04 & 23.18 & 0.04 & 23.13 & 0.02 & 22.78 & 0.04 & 1.0 & 2.0 & 2814.34 & 1226.26 & 0.38 & 0.05 & -1.45 & 2.0\\
  55.519661\_-47.205105 & ngc1433 & 55.51966 & -47.2051 & 4580.52 & 6490.87 & 21.24 & 0.03 & 21.6 & 0.03 & 22.92 & 0.03 & 23.01 & 0.02 & 22.98 & 0.04 & 3.0 & 2.0 & 1283.95 & 852.85 & 0.23 & 0.19 & -1.65 & 3.0\\
  55.470708\_-47.222587 & ngc1433 & 55.47071 & -47.22259 & 7602.19 & 4901.95 & 22.67 & 0.1 & 22.75 & 0.09 & 23.13 & 0.04 & 22.54 & 0.02 & 21.57 & 0.02 & 49.0 & 6.0 & 12905.63 & 2686.09 & 0.4 & 0.04 & -1.72 & 3.0\\
  55.488599\_-47.228569 & ngc1433 & 55.4886 & -47.22857 & 6498.08 & 4358.07 & 21.93 & 0.05 & 22.23 & 0.06 & 23.68 & 0.06 & 23.69 & 0.04 & 23.37 & 0.07 & 1.0 & 6.0 & 1347.84 & 1076.21 & 0.3 & 0.28 & -0.91 & 3.0\\
  55.526279\_-47.212308 & ngc1433 & 55.52628 & -47.21231 & 4172.77 & 5837.36 & 20.59 & 0.03 & 21.14 & 0.04 & 22.63 & 0.04 & 22.74 & 0.03 & 22.81 & 0.08 & 1.0 & 1.0 & 1847.16 & 82.5 & 0.14 & 0.04 & -0.71 & 3.0\\
  55.541609\_-47.228118 & ngc1433 & 55.54161 & -47.22812 & 3226.25 & 4399.1 & 21.32 & 0.03 & 21.73 & 0.04 & 23.14 & 0.04 & 23.05 & 0.02 & 22.32 & 0.03 & 9.0 & 1.0 & 738.39 & 164.74 & 0.0 & 0.01 & -1.78 & 3.0\\
  55.47162\_-47.220467 & ngc1433 & 55.47162 & -47.22047 & 7546.38 & 5094.38 & 21.4 & 0.04 & 21.75 & 0.04 & 23.23 & 0.05 & 23.16 & 0.04 & 22.82 & 0.06 & 1.0 & 6.0 & 2163.26 & 1708.72 & 0.3 & 0.27 & -1.22 & 3.0\\
  55.545681\_-47.225093 & ngc1433 & 55.54568 & -47.22509 & 2975.81 & 4674.32 & 23.16 & 0.15 & 23.32 & 0.14 & 24.3 & 0.1 & 24.2 & 0.06 & 23.83 & 0.12 & 4.0 & 28.0 & 410.35 & 376.58 & 0.39 & 0.35 & -0.74 & 3.0\\
  64.439237\_-62.770925 & ngc1559 & 64.43924 & -62.77092 & 1920.04 & 4629.06 & 23.53 & 0.13 & 22.16 & 0.05 & 21.96 & 0.01 & 21.25 & 0.01 & 19.85 & 0.0 & 2440.0 & 1335.0 & 1546440.57 & 557168.71 & 0.07 & 0.14 & -1.5 & 1.0\\
  64.382767\_-62.770983 & ngc1559 & 64.38277 & -62.77098 & 4267.63 & 4623.99 & 23.71 & 0.17 & 22.76 & 0.09 & 22.9 & 0.03 & 22.33 & 0.01 & 21.28 & 0.01 & 182.0 & 55.0 & 207766.16 & 905.26 & 0.44 & 0.08 & -1.51 & 1.0\\
  64.382884\_-62.769244 & ngc1559 & 64.38288 & -62.76924 & 4262.92 & 4782.1 & 24.35 & 0.3 & 23.23 & 0.13 & 23.02 & 0.03 & 22.37 & 0.01 & 21.21 & 0.01 & 1276.0 & 448.0 & 269915.11 & 21142.5 & 0.07 & 0.09 & -1.41 & 1.0\\
  64.435287\_-62.764827 & ngc1559 & 64.43529 & -62.76483 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & -1.46 & 1.0\\
  64.439639\_-62.769921 & ngc1559 & 64.43964 & -62.76992 & 1903.11 & 4720.22 & 22.65 & 0.06 & 22.45 & 0.07 & 22.57 & 0.02 & 22.39 & 0.01 & 21.77 & 0.01 & 243.0 & 61.0 & 72253.96 & 1357.3 & 0.05 & 0.05 & -1.64 & 1.0\\
  64.417324\_-62.767447 & ngc1559 & 64.41732 & -62.76745 & 2830.83 & 4945.39 & 24.6 & 0.33 & 23.74 & 0.21 & 23.99 & 0.07 & 23.36 & 0.02 & 22.19 & 0.01 & 5.0 & 113.0 & 23624.53 & 76817.6 & 0.93 & 0.33 & -1.33 & 1.0\\
  64.454279\_-62.782222 & ngc1559 & 64.45428 & -62.78222 & 1295.44 & 3602.14 & 22.74 & 0.08 & 22.39 & 0.06 & 22.82 & 0.03 & 22.64 & 0.01 & 21.99 & 0.01 & 169.0 & 13.0 & 55867.98 & 5747.1 & 0.1 & 0.05 & -1.51 & 1.0\\
  64.397357\_-62.76776 & ngc1559 & 64.39736 & -62.76776 & 3661.15 & 4916.98 & 23.98 & 0.2 & 23.62 & 0.18 & 23.44 & 0.04 & 23.09 & 0.01 & 22.34 & 0.01 & 349.0 & 153.0 & 57724.11 & 207.88 & 0.12 & 0.12 & -1.48 & 1.0\\
  64.436693\_-62.78119 & ngc1559 & 64.43669 & -62.78119 & 2026.12 & 3696.49 & 23.09 & 0.1 & 22.32 & 0.06 & 22.13 & 0.02 & 21.74 & 0.01 & 20.68 & 0.01 & 324.0 & 141.0 & 314357.2 & 73356.44 & 0.27 & 0.03 & -1.7 & 1.0\\
  64.406131\_-62.789846 & ngc1559 & 64.40613 & -62.78985 & 3296.34 & 2910.31 & 22.55 & 0.07 & 21.98 & 0.05 & 21.77 & 0.01 & 21.54 & 0.01 & 20.7 & 0.01 & 465.0 & 116.0 & 274849.12 & 22842.72 & 0.07 & 0.1 & -1.74 & 1.0\\
  64.432702\_-62.795627 & ngc1559 & 64.4327 & -62.79563 & 2192.66 & 2384.74 & 23.82 & 0.18 & 22.79 & 0.09 & 22.69 & 0.02 & 22.18 & 0.01 & 21.06 & 0.01 & 1276.0 & 1094.0 & 272555.09 & 8499.01 & 0.0 & 0.49 & -1.59 & 1.0\\
  64.453074\_-62.783311 & ngc1559 & 64.45307 & -62.78331 & 1345.61 & 3503.17 & 22.61 & 0.07 & 22.41 & 0.07 & 22.7 & 0.02 & 22.63 & 0.01 & 22.1 & 0.01 & 210.0 & 52.0 & 48870.51 & 602.68 & 0.01 & 0.06 & -1.54 & 1.0\\
  64.398478\_-62.773086 & ngc1559 & 64.39848 & -62.77309 & 3614.67 & 4432.8 & 20.5 & 0.01 & 20.79 & 0.02 & 22.43 & 0.02 & 21.97 & 0.01 & 22.08 & 0.02 & 1.0 & 1.0 & 26374.29 & 8110.4 & 0.3 & 0.04 & -1.63 & 2.0\\
  64.429915\_-62.782535 & ngc1559 & 64.42992 & -62.78254 & 2307.95 & 3574.4 & 20.53 & 0.02 & 20.5 & 0.02 & 21.62 & 0.02 & 21.07 & 0.01 & 20.15 & 0.01 & 19.0 & 10.0 & 106320.68 & 55629.33 & 0.28 & 0.02 & -1.71 & 2.0\\
  64.372437\_-62.791413 & ngc1559 & 64.37244 & -62.79141 & 4696.34 & 2767.48 & 22.08 & 0.05 & 21.98 & 0.05 & 23.35 & 0.04 & 22.88 & 0.02 & 22.71 & 0.03 & 2.0 & 1.0 & 17942.19 & 1746.84 & 0.5 & 0.02 & -1.5 & 2.0\\
  64.36884\_-62.790919 & ngc1559 & 64.36884 & -62.79092 & 4845.83 & 2811.62 & 22.47 & 0.06 & 22.18 & 0.06 & 23.65 & 0.06 & 23.14 & 0.03 & 22.66 & 0.03 & 1.0 & 2.0 & 25291.15 & 10856.79 & 0.59 & 0.05 & -1.65 & 2.0\\
  64.391368\_-62.795462 & ngc1559 & 64.39137 & -62.79546 & 3909.83 & 2399.77 & 21.14 & 0.02 & 21.63 & 0.04 & 23.16 & 0.04 & 22.98 & 0.02 & 22.99 & 0.03 & 1.0 & 2.0 & 10003.44 & 2886.34 & 0.24 & 0.01 & -1.47 & 2.0\\
  64.427684\_-62.777434 & ngc1559 & 64.42768 & -62.77743 & 2400.38 & 4037.83 & 18.46 & 0.01 & 18.72 & 0.01 & 20.04 & 0.01 & 20.04 & 0.01 & 19.66 & 0.02 & 1.0 & 1.0 & 249368.16 & 22747.22 & 0.36 & 0.03 & -1.64 & 2.0\\
  64.427243\_-62.782743 & ngc1559 & 64.42724 & -62.78274 & 2419.04 & 3555.42 & 17.76 & 0.01 & 17.98 & 0.01 & 19.24 & 0.01 & 19.28 & 0.01 & 18.92 & 0.01 & 1.0 & 0.0 & 518346.84 & 58067.85 & 0.37 & 0.03 & -1.7 & 2.0\\
  64.381358\_-62.797968 & ngc1559 & 64.38136 & -62.79797 & 4325.58 & 2171.64 & 19.88 & 0.02 & 20.2 & 0.02 & 21.68 & 0.02 & 21.04 & 0.01 & 20.97 & 0.01 & 1.0 & 1.0 & 86103.31 & 26369.53 & 0.42 & 0.04 & -1.46 & 2.0\\
  64.378677\_-62.792617 & ngc1559 & 64.37868 & -62.79262 & 4437.08 & 2658.33 & 19.76 & 0.01 & 20.37 & 0.02 & 21.73 & 0.02 & 21.91 & 0.02 & 21.82 & 0.02 & 1.0 & 2.0 & 25200.99 & 11008.16 & 0.18 & 0.05 & -1.46 & 3.0\\
  64.378351\_-62.798943 & ngc1559 & 64.37835 & -62.79894 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & -0.68 & 3.0\\
  64.383545\_-62.792137 & ngc1559 & 64.38354 & -62.79214 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & -1.1 & 3.0\\
  64.407594\_-62.771456 & ngc1559 & 64.40759 & -62.77146 & 3235.48 & 4581.13 & 19.59 & 0.02 & 20.16 & 0.02 & 21.48 & 0.02 & 21.3 & 0.02 & 20.58 & 0.01 & 10.0 & 1.0 & 21997.03 & 338.68 & 0.0 & 0.04 & -1.63 & 3.0\\
  64.423919\_-62.776378 & ngc1559 & 64.42392 & -62.77638 & 2556.81 & 4133.76 & 19.3 & 0.02 & 19.73 & 0.02 & 21.05 & 0.02 & 21.09 & 0.02 & 20.72 & 0.01 & 7.0 & 0.0 & 14774.56 & 1782.03 & 0.0 & 0.03 & -0.95 & 3.0\\
  64.398308\_-62.774084 & ngc1559 & 64.39831 & -62.77408 & 3621.64 & 4342.31 & 20.17 & 0.02 & 20.76 & 0.03 & 22.32 & 0.04 & 22.48 & 0.05 & 21.79 & 0.04 & 8.0 & 7.0 & 6211.98 & 12701.3 & 0.0 & 0.21 & -0.91 & 3.0\\
  64.385496\_-62.791729 & ngc1559 & 64.3855 & -62.79173 & 4153.96 & 2738.79 & 20.42 & 0.04 & 20.69 & 0.05 & 21.77 & 0.04 & 21.77 & 0.06 & 21.51 & 0.07 & 4.0 & 3.0 & 15223.37 & 47284.73 & 0.29 & 0.15 & -0.72 & 3.0\\
  64.412183\_-62.77377 & ngc1559 & 64.41218 & -62.77377 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & -0.82 & 3.0\\
  64.412178\_-62.773769 & ngc1559 & 64.41218 & -62.77377 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & -0.82 & 3.0\\
  64.391501\_-62.791735 & ngc1559 & 64.3915 & -62.79174 & 3904.23 & 2738.39 & 19.88 & 0.01 & 19.77 & 0.01 & 19.88 & 0.01 & 19.64 & 0.0 & 18.74 & 0.0 & 136.0 & 34.0 & 1255326.75 & 117809.45 & 0.25 & 0.03 & -1.78 & 1.0\\
  64.428196\_-62.788606 & ngc1559 & 64.4282 & -62.78861 & 2379.69 & 3022.76 & 21.32 & 0.03 & 21.4 & 0.03 & 22.77 & 0.03 & 22.1 & 0.01 & 21.99 & 0.01 & 2.0 & 1.0 & 33126.99 & 9086.97 & 0.5 & 0.04 & -1.72 & 1.0\\
  64.413724\_-62.785114 & ngc1559 & 64.41372 & -62.78511 & 2980.94 & 3340.22 & 20.84 & 0.02 & 20.82 & 0.02 & 21.04 & 0.01 & 20.94 & 0.01 & 20.27 & 0.01 & 158.0 & 68.0 & 244134.64 & 15171.8 & 0.08 & 0.06 & -1.7 & 1.0\\
  64.416867\_-62.784495 & ngc1559 & 64.41687 & -62.78449 & 2850.33 & 3396.3 & 19.99 & 0.01 & 20.29 & 0.02 & 21.18 & 0.01 & 21.2 & 0.01 & 20.58 & 0.01 & 37.0 & 5.0 & 72943.31 & 8155.93 & 0.02 & 0.05 & -1.75 & 1.0\\
  64.374055\_-62.779935 & ngc1559 & 64.37406 & -62.77993 & 4629.54 & 3810.58 & 21.41 & 0.03 & 21.53 & 0.03 & 21.85 & 0.01 & 21.69 & 0.01 & 21.1 & 0.01 & 136.0 & 11.0 & 102203.89 & 14149.96 & 0.06 & 0.02 & -1.71 & 1.0\\
  64.441673\_-62.776296 & ngc1559 & 64.44167 & -62.7763 & 1818.98 & 4140.82 & 20.97 & 0.02 & 20.96 & 0.02 & 21.29 & 0.01 & 21.14 & 0.01 & 20.42 & 0.01 & 118.0 & 9.0 & 219176.17 & 18535.84 & 0.15 & 0.01 & -1.75 & 1.0\\
  64.978957\_-54.929273 & ngc1566 & 64.97896 & -54.92927 & 4878.03 & 4438.04 & 22.49 & 0.07 & 22.24 & 0.05 & 22.34 & 0.02 & 22.13 & 0.01 & 21.49 & 0.02 & 243.0 & 81.0 & 85866.45 & 2175.57 & 0.07 & 0.06 & -1.7 & 1.0\\
  65.001972\_-54.925844 & ngc1566 & 65.00197 & -54.92584 & 3676.26 & 4749.89 & 23.38 & 0.15 & 22.71 & 0.08 & 22.36 & 0.02 & 22.15 & 0.01 & 21.41 & 0.02 & 577.0 & 0.0 & 126302.18 & 20849.01 & 0.0 & 0.05 & -1.69 & 1.0\\
  64.997862\_-54.917984 & ngc1566 & 64.99786 & -54.91798 & 3891.25 & 5463.91 & 22.51 & 0.07 & 22.26 & 0.05 & 22.1 & 0.02 & 21.87 & 0.01 & 21.09 & 0.01 & 302.0 & 131.0 & 138350.94 & 18102.43 & 0.1 & 0.06 & -1.68 & 1.0\\
  65.0006\_-54.915616 & ngc1566 & 65.0006 & -54.91562 & 3748.09 & 5679.13 & 22.65 & 0.08 & 22.37 & 0.05 & 22.36 & 0.02 & 21.94 & 0.01 & 21.01 & 0.01 & 169.0 & 42.0 & 178062.75 & 12516.82 & 0.32 & 0.08 & -1.58 & 1.0\\
  65.013583\_-54.914897 & ngc1566 & 65.01358 & -54.9149 & 3070.09 & 5744.5 & 21.58 & 0.03 & 21.57 & 0.03 & 21.93 & 0.02 & 21.83 & 0.01 & 21.34 & 0.01 & 169.0 & 51.0 & 76358.9 & 2130.82 & 0.0 & 0.08 & -1.56 & 1.0\\
  65.003868\_-54.915414 & ngc1566 & 65.00387 & -54.91541 & 3577.29 & 5697.51 & 20.89 & 0.02 & 20.67 & 0.02 & 20.82 & 0.01 & 20.56 & 0.01 & 19.86 & 0.01 & 196.0 & 38.0 & 421385.44 & 16917.08 & 0.15 & 0.06 & -1.74 & 1.0\\
  65.032265\_-54.92893 & ngc1566 & 65.03226 & -54.92893 & 2094.9 & 4469.16 & 19.79 & 0.01 & 20.03 & 0.01 & 20.66 & 0.01 & 20.55 & 0.0 & 20.02 & 0.01 & 82.0 & 25.0 & 177421.98 & 263.65 & 0.02 & 0.07 & -1.61 & 1.0\\
  64.994227\_-54.936213 & ngc1566 & 64.99423 & -54.93621 & 4080.71 & 3807.51 & 22.64 & 0.08 & 22.33 & 0.06 & 22.23 & 0.02 & 22.01 & 0.01 & 21.35 & 0.02 & 375.0 & 94.0 & 108064.07 & 8253.98 & 0.01 & 0.1 & -1.76 & 1.0\\
  64.97778\_-54.936421 & ngc1566 & 64.97778 & -54.93642 & 4939.04 & 3788.58 & 21.34 & 0.03 & 21.33 & 0.03 & 21.46 & 0.01 & 21.32 & 0.01 & 20.74 & 0.01 & 226.0 & 16.0 & 153028.84 & 13589.44 & 0.02 & 0.01 & -1.72 & 1.0\\
  64.976169\_-54.937217 & ngc1566 & 64.97617 & -54.93722 & 5023.39 & 3716.35 & 22.31 & 0.06 & 22.19 & 0.05 & 21.98 & 0.02 & 21.72 & 0.01 & 21.08 & 0.01 & 324.0 & 63.0 & 136746.48 & 2507.53 & 0.05 & 0.05 & -1.62 & 1.0\\
  65.008335\_-54.934174 & ngc1566 & 65.00834 & -54.93417 & 3344.37 & 3992.93 & 26.58 & 3.57 & 23.2 & 0.15 & 22.86 & 0.05 & 21.94 & 0.01 & 20.64 & 0.01 & 8304.0 & 7028.0 & 1432660.64 & 938062.91 & 0.0 & 0.2 & -1.88 & 1.0\\
  64.9956\_-54.94891 & ngc1566 & 64.9956 & -54.94891 & 4009.25 & 2654.05 & 20.22 & 0.01 & 20.69 & 0.02 & 22.28 & 0.02 & 22.29 & 0.01 & 22.33 & 0.04 & 1.0 & 0.0 & 13797.12 & 2343.99 & 0.16 & 0.04 & -1.75 & 2.0\\
  64.991385\_-54.91861 & ngc1566 & 64.99138 & -54.91861 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & -1.23 & 2.0\\
  64.999835\_-54.946484 & ngc1566 & 64.99984 & -54.94648 & 3787.99 & 2874.15 & 19.28 & 0.01 & 19.86 & 0.01 & 21.38 & 0.02 & 21.52 & 0.01 & 21.57 & 0.03 & 1.0 & 0.0 & 26676.52 & 3282.82 & 0.13 & 0.03 & -1.48 & 2.0\\
  65.023479\_-54.945715 & ngc1566 & 65.02348 & -54.94572 & 2554.01 & 2944.15 & 17.93 & 0.02 & 18.38 & 0.02 & 19.83 & 0.02 & 19.88 & 0.02 & 19.81 & 0.02 & 1.0 & 1.0 & 158797.94 & 48853.08 & 0.22 & 0.04 & -1.06 & 2.0\\
  64.980302\_-54.931479 & ngc1566 & 64.9803 & -54.93148 & 4807.77 & 4237.72 & 17.69 & 0.01 & 18.13 & 0.01 & 19.3 & 0.01 & 19.33 & 0.01 & 18.63 & 0.01 & 19.0 & 8.0 & 237252.05 & 101938.38 & 0.0 & 0.01 & -1.76 & 2.0\\
  64.997169\_-54.946122 & ngc1566 & 64.99717 & -54.94612 & 3927.12 & 2907.28 & 18.04 & 0.0 & 18.5 & 0.0 & 19.75 & 0.0 & 19.71 & 0.0 & 19.32 & 0.0 & 8.0 & 0.0 & 53964.24 & 6489.57 & 0.0 & 0.03 & -1.73 & 2.0\\
  65.002407\_-54.913111 & ngc1566 & 65.00241 & -54.91311 & 3653.62 & 5907.21 & 20.0 & 0.02 & 20.49 & 0.02 & 22.08 & 0.02 & 22.12 & 0.02 & 22.02 & 0.03 & 1.0 & 2.0 & 18176.33 & 7948.98 & 0.18 & 0.05 & -1.71 & 2.0\\
  65.012209\_-54.941023 & ngc1566 & 65.01221 & -54.94102 & 3142.17 & 3370.6 & 16.89 & 0.0 & 17.39 & 0.0 & 18.75 & 0.0 & 18.8 & 0.0 & 18.49 & 0.0 & 7.0 & 4.0 & 110578.3 & 237231.5 & 0.0 & 0.26 & -1.75 & 2.0\\
  65.012098\_-54.942276 & ngc1566 & 65.0121 & -54.94228 & 3148.11 & 3256.8 & 18.32 & 0.01 & 18.8 & 0.01 & 20.29 & 0.01 & 20.37 & 0.01 & 20.35 & 0.01 & 1.0 & 0.0 & 88958.45 & 10073.63 & 0.18 & 0.03 & -1.63 & 2.0\\
  64.985653\_-54.932999 & ngc1566 & 64.98565 & -54.933 & 4529.04 & 4099.65 & 19.38 & 0.01 & 19.73 & 0.01 & 20.67 & 0.01 & 20.64 & 0.0 & 19.98 & 0.01 & 32.0 & 25.0 & 109026.62 & 72827.98 & 0.04 & 0.15 & -1.69 & 2.0\\
  65.009181\_-54.943822 & ngc1566 & 65.00918 & -54.94382 & 3300.4 & 3116.45 & 19.58 & 0.06 & 19.82 & 0.04 & 21.22 & 0.04 & 21.3 & 0.05 & 20.99 & 0.08 & 1.0 & 0.0 & 58219.16 & 12544.97 & 0.3 & 0.05 & -1.17 & 3.0\\
  64.990715\_-54.921256 & ngc1566 & 64.99072 & -54.92126 & 4264.62 & 5167.08 & 19.14 & 0.06 & 19.69 & 0.06 & 21.2 & 0.06 & 21.33 & 0.05 & 21.4 & 0.06 & 1.0 & 2.0 & 31160.84 & 7188.02 & 0.13 & 0.03 & -1.04 & 3.0\\
  64.982862\_-54.930516 & ngc1566 & 64.98286 & -54.93052 & 4674.29 & 4325.2 & 18.33 & 0.01 & 18.88 & 0.02 & 20.47 & 0.02 & 20.5 & 0.02 & 20.33 & 0.03 & 1.0 & 1.0 & 81792.05 & 7244.89 & 0.18 & 0.03 & -1.67 & 3.0\\
  64.986738\_-54.933937 & ngc1566 & 64.98674 & -54.93394 & 4471.84 & 4014.34 & 23.67 & 0.3 & 23.56 & 0.22 & 24.8 & 0.26 & 24.12 & 0.12 & 23.4 & 0.15 & 1.0 & 12.0 & 14271.7 & 11981.91 & 0.73 & 0.57 & -0.53 & 3.0\\
  64.97996\_-54.928893 & ngc1566 & 64.97996 & -54.92889 & 4825.56 & 4472.87 & 19.75 & 0.02 & 20.26 & 0.02 & 21.86 & 0.02 & 21.94 & 0.02 & 21.81 & 0.03 & 1.0 & 1.0 & 20495.73 & 1802.97 & 0.16 & 0.03 & -1.86 & 3.0\\
  65.040718\_-54.932727 & ngc1566 & 65.04072 & -54.93273 & 1653.85 & 4123.88 & 20.14 & 0.02 & 20.66 & 0.02 & 22.13 & 0.03 & 22.15 & 0.03 & 21.75 & 0.03 & 1.0 & 0.0 & 23963.64 & 4000.82 & 0.26 & 0.04 & -0.56 & 3.0\\
  64.989798\_-54.945088 & ngc1566 & 64.9898 & -54.94509 & 4311.65 & 3000.47 & 21.05 & 0.04 & 21.59 & 0.05 & 22.82 & 0.05 & 22.87 & 0.04 & 22.92 & 0.08 & 4.0 & 3.0 & 2751.74 & 6496.94 & 0.12 & 0.1 & -0.95 & 3.0\\
  64.991593\_-54.946104 & ngc1566 & 64.99159 & -54.9461 & 4218.46 & 2908.84 & 21.64 & 0.07 & 21.91 & 0.06 & 22.81 & 0.05 & 22.58 & 0.03 & 22.05 & 0.04 & 7.0 & 25.0 & 6511.11 & 10356.09 & 0.25 & 0.19 & -0.64 & 3.0\\
  64.995311\_-54.954663 & ngc1566 & 64.99531 & -54.95466 & 4024.04 & 2131.22 & 19.31 & 0.01 & 19.49 & 0.01 & 20.16 & 0.01 & 20.06 & 0.0 & 19.5 & 0.01 & 76.0 & 23.0 & 290089.4 & 10276.06 & 0.04 & 0.06 & -1.71 & 1.0\\
  64.989264\_-54.94197 & ngc1566 & 64.98926 & -54.94197 & 4339.73 & 3284.43 & 21.17 & 0.02 & 21.3 & 0.03 & 21.8 & 0.02 & 21.69 & 0.01 & 21.13 & 0.01 & 102.0 & 20.0 & 77299.83 & 9256.56 & 0.05 & 0.01 & -1.69 & 1.0\\
  65.022229\_-54.941314 & ngc1566 & 65.02223 & -54.94131 & 2619.2 & 3344.12 & 18.93 & 0.01 & 19.38 & 0.01 & 20.68 & 0.01 & 20.66 & 0.01 & 20.22 & 0.01 & 8.0 & 0.0 & 23333.82 & 1837.39 & 0.0 & 0.02 & -1.7 & 1.0\\
  65.016952\_-54.940424 & ngc1566 & 65.01695 & -54.94042 & 2894.19 & 3425.08 & 20.33 & 0.01 & 20.7 & 0.02 & 21.49 & 0.01 & 21.44 & 0.01 & 20.94 & 0.01 & 53.0 & 4.0 & 58780.32 & 120.62 & 0.0 & 0.02 & -1.81 & 1.0\\
  65.029535\_-54.93713 & ngc1566 & 65.02954 & -54.93713 & 2237.76 & 3724.09 & 20.23 & 0.01 & 20.56 & 0.02 & 21.46 & 0.01 & 21.38 & 0.01 & 20.69 & 0.01 & 32.0 & 11.0 & 59535.35 & 4987.54 & 0.07 & 0.07 & -1.48 & 1.0\\
  76.315541\_-37.965588 & ngc1792 & 76.31554 & -37.96559 & 2969.07 & 5007.24 & 24.98 & 0.78 & 24.14 & 0.32 & 24.07 & 0.09 & 23.38 & 0.04 & 22.03 & 0.03 & 118.0 & 2322.0 & 82592.73 & 46350.42 & 0.65 & 0.63 & -1.55 & 1.0\\
  76.312082\_-37.975889 & ngc1792 & 76.31208 & -37.97589 & 3216.52 & 4071.1 & 19.37 & 0.01 & 19.49 & 0.01 & 20.29 & 0.01 & 20.21 & 0.01 & 19.46 & 0.01 & 7.0 & 36.0 & 57770.34 & 95292.98 & 0.3 & 0.23 & -1.71 & 1.0\\
  76.311089\_-37.967832 & ngc1792 & 76.31109 & -37.96783 & 3287.65 & 4803.01 & 23.58 & 0.25 & 22.85 & 0.11 & 22.42 & 0.03 & 22.06 & 0.02 & 21.22 & 0.02 & 537.0 & 37.0 & 138519.64 & 28112.01 & 0.11 & 0.08 & -1.64 & 1.0\\
  76.332561\_-37.977069 & ngc1792 & 76.33256 & -37.97707 & 1749.43 & 3963.36 &  & -1.58 & 24.02 & 0.28 & 23.66 & 0.06 & 22.8 & 0.03 & 21.42 & 0.02 & 1276.0 & 506.0 & 211412.77 & 73094.77 & 0.25 & 0.25 & -1.62 & 1.0\\
  76.276558\_-37.987693 & ngc1792 & 76.27656 & -37.98769 & 5760.55 & 2998.03 & 23.01 & 0.13 & 22.29 & 0.06 & 22.38 & 0.02 & 21.76 & 0.01 & 20.64 & 0.01 & 118.0 & 18.0 & 248929.55 & 25528.85 & 0.53 & 0.01 & -1.6 & 1.0\\
  76.311933\_-37.996675 & ngc1792 & 76.31193 & -37.99668 & 3227.15 & 2182.33 &  & -1.98 & 23.15 & 0.13 & 22.62 & 0.03 & 21.62 & 0.01 & 20.07 & 0.01 & 1474.0 & 7451.0 & 1110530.28 & 979019.07 & 0.39 & 0.31 & -1.62 & 1.0\\
  76.302217\_-37.99667 & ngc1792 & 76.30222 & -37.99667 & 3922.82 & 2182.87 & 25.45 & 1.26 & 23.54 & 0.18 & 23.47 & 0.05 & 22.55 & 0.02 & 21.12 & 0.02 & 2440.0 & 2197.0 & 419783.22 & 135914.31 & 0.18 & 0.52 & -1.55 & 1.0\\
  76.314378\_-37.994844 & ngc1792 & 76.31438 & -37.99484 & 3052.12 & 2348.68 & 23.23 & 0.18 & 23.04 & 0.12 & 22.93 & 0.04 & 22.4 & 0.02 & 21.43 & 0.02 & 169.0 & 67.0 & 108791.46 & 6701.16 & 0.39 & 0.08 & -1.74 & 1.0\\
  76.292015\_-37.963238 & ngc1792 & 76.29202 & -37.96324 & 4653.68 & 5220.64 & 23.5 & 0.25 & 23.48 & 0.18 & 23.33 & 0.05 & 22.65 & 0.03 & 21.72 & 0.03 & 182.0 & 167.0 & 93895.87 & 10321.15 & 0.42 & 0.17 & -1.56 & 1.0\\
  76.325463\_-37.984056 & ngc1792 & 76.32546 & -37.98406 & 2258.12 & 3329.2 & 20.67 & 0.02 & 20.59 & 0.02 & 21.19 & 0.01 & 21.05 & 0.01 & 20.39 & 0.01 & 5.0 & 66.0 & 40062.29 & 91803.08 & 0.5 & 0.33 & -1.71 & 1.0\\
  76.298839\_-37.96627 & ngc1792 & 76.29884 & -37.96627 & 4165.17 & 4945.23 & 17.54 & 0.01 & 17.84 & 0.01 & 18.8 & 0.01 & 18.77 & 0.01 & 18.13 & 0.01 & 32.0 & 0.0 & 472984.94 & 56514.68 & 0.04 & 0.03 & -1.69 & 2.0\\
  76.304545\_-37.965406 & ngc1792 & 76.30454 & -37.96541 & 3756.18 & 5023.74 & 22.1 & 0.07 & 21.74 & 0.05 & 21.63 & 0.02 & 21.24 & 0.01 & 20.33 & 0.01 & 226.0 & 68.0 & 276953.49 & 12961.4 & 0.28 & 0.09 & -1.7 & 2.0\\
  76.302039\_-37.968732 & ngc1792 & 76.30204 & -37.96873 & 3936.09 & 4721.73 & 18.56 & 0.01 & 18.86 & 0.01 & 19.74 & 0.01 & 19.71 & 0.01 & 19.13 & 0.01 & 43.0 & 37.0 & 197208.87 & 133874.96 & 0.0 & 0.23 & -1.66 & 2.0\\
  76.314312\_-37.973039 & ngc1792 & 76.31431 & -37.97304 & 3056.59 & 4330.3 & 18.87 & 0.01 & 18.89 & 0.01 & 20.05 & 0.01 & 19.93 & 0.01 & 19.53 & 0.01 & 1.0 & 2.0 & 270004.33 & 77711.21 & 0.49 & 0.01 & -1.66 & 2.0\\
  76.323597\_-37.982193 & ngc1792 & 76.3236 & -37.98219 & 2391.57 & 3498.22 & 20.2 & 0.02 & 20.26 & 0.02 & 20.95 & 0.01 & 20.78 & 0.01 & 20.17 & 0.01 & 71.0 & 10.0 & 134087.57 & 24488.93 & 0.1 & 0.02 & -1.6 & 2.0\\
  76.306096\_-37.999162 & ngc1792 & 76.3061 & -37.99916 & 3645.25 & 1956.38 & 24.83 & 0.7 & 24.15 & 0.3 & 23.75 & 0.06 & 23.07 & 0.03 & 21.75 & 0.02 & 243.0 & 1459.0 & 122216.26 & 67927.52 & 0.56 & 0.37 & -1.47 & 2.0\\
  76.316952\_-37.980437 & ngc1792 & 76.31695 & -37.98044 & 2867.57 & 3657.14 & 23.71 & 0.28 & 23.15 & 0.14 & 22.54 & 0.03 & 22.2 & 0.02 & 21.26 & 0.03 & 465.0 & 305.0 & 147363.22 & 8580.31 & 0.2 & 0.15 & -1.49 & 2.0\\
  76.309005\_-37.970753 & ngc1792 & 76.309 & -37.97075 & 3436.71 & 4537.95 & 18.57 & 0.01 & 18.59 & 0.01 & 19.79 & 0.01 & 19.47 & 0.01 & 18.79 & 0.01 & 1.0 & 6.0 & 574830.89 & 479294.53 & 0.59 & 0.33 & -1.69 & 2.0\\
  76.294779\_-37.971346 & ngc1792 & 76.29478 & -37.97135 & 4455.81 & 4483.88 & 20.57 & 0.03 & 20.54 & 0.02 & 21.18 & 0.02 & 20.98 & 0.01 & 20.07 & 0.02 & 46.0 & 12.0 & 130408.05 & 15525.49 & 0.23 & 0.02 & -1.64 & 2.0\\
  76.322263\_-37.981733 & ngc1792 & 76.32226 & -37.98173 & 2487.18 & 3539.49 & 20.42 & 0.06 & 20.31 & 0.04 & 21.23 & 0.03 & 21.07 & 0.03 & 20.54 & 0.03 & 4.0 & 3.0 & 38238.4 & 81680.93 & 0.5 & 0.08 & -1.81 & 3.0\\
  76.315175\_-37.980681 & ngc1792 & 76.31518 & -37.98068 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & -1.02 & 3.0\\
  76.317242\_-37.986908 & ngc1792 & 76.31724 & -37.98691 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & -0.9 & 3.0\\
  76.318103\_-37.992288 & ngc1792 & 76.3181 & -37.99229 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & -1.42 & 3.0\\
  76.319395\_-37.992495 & ngc1792 & 76.3194 & -37.9925 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & -0.99 & 3.0\\
  76.315856\_-37.973799 & ngc1792 & 76.31586 & -37.9738 & 2946.81 & 4261.16 & 23.07 & 0.2 & 22.99 & 0.19 & 23.5 & 0.11 & 22.96 & 0.06 & 21.96 & 0.06 & 6.0 & 47.0 & 10150.49 & 33746.02 & 0.64 & 0.17 & -1.28 & 3.0\\
  76.311765\_-37.972071 & ngc1792 & 76.31177 & -37.97207 & 3239.4 & 4418.71 & 21.06 & 0.07 & 21.23 & 0.07 & 21.99 & 0.06 & 21.71 & 0.05 & 20.83 & 0.06 & 32.0 & 14.0 & 54237.13 & 5705.32 & 0.23 & 0.09 & -0.8 & 3.0\\
  76.309084\_-37.969391 & ngc1792 & 76.30908 & -37.96939 & 3431.34 & 4660.94 & 20.55 & 0.05 & 20.86 & 0.06 & 22.08 & 0.05 & 22.03 & 0.05 & 21.9 & 0.07 & 3.0 & 2.0 & 15452.23 & 9853.74 & 0.33 & 0.17 & -1.09 & 3.0\\
  76.301909\_-37.968406 & ngc1792 & 76.30191 & -37.96841 & 3945.44 & 4751.68 & 20.39 & 0.05 & 20.49 & 0.03 & 21.34 & 0.02 & 21.08 & 0.02 & 19.88 & 0.01 & 19.0 & 9.0 & 94732.12 & 39326.72 & 0.31 & 0.03 & -1.4 & 3.0\\
  76.300709\_-37.965346 & ngc1792 & 76.30071 & -37.96535 & 4030.36 & 5029.47 & 19.59 & 0.02 & 20.06 & 0.02 & 21.58 & 0.02 & 21.72 & 0.02 & 21.83 & 0.05 & 1.0 & 1.0 & 17467.75 & 5449.99 & 0.14 & 0.04 & -1.68 & 3.0\\
  137.585641\_7.036904 & ngc2775 & 137.58564 & 7.0369 & 3862.32 & 3732.23 & 22.82 & 0.11 & 22.05 & 0.05 & 22.01 & 0.02 & 21.42 & 0.01 & 20.36 & 0.02 & 196.0 & 832.0 & 731623.04 & 47753.64 & 0.45 & 0.42 & -1.67 & 1.0\\
  137.587942\_7.064121 & ngc2775 & 137.58794 & 7.06412 & 3654.9 & 6205.26 & 23.47 & 0.16 & 21.75 & 0.03 & 21.38 & 0.01 & 20.55 & 0.01 & 19.22 & 0.01 & 7727.0 & 3686.0 & 8054687.38 & 2710496.15 & 0.0 & 0.04 & -1.69 & 1.0\\
  137.590965\_7.019892 & ngc2775 & 137.59096 & 7.01989 & 3382.23 & 2186.91 & 22.93 & 0.11 & 22.36 & 0.05 & 22.53 & 0.02 & 21.94 & 0.01 & 20.88 & 0.01 & 110.0 & 48.0 & 358050.69 & 37620.58 & 0.48 & 0.1 & -1.55 & 1.0\\
  137.58557\_7.039144 & ngc2775 & 137.58557 & 7.03914 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & -1.59 & 1.0\\
  137.592478\_7.041045 & ngc2775 & 137.59248 & 7.04104 & 3245.75 & 4108.43 & 23.29 & 0.16 & 22.69 & 0.07 & 22.6 & 0.02 & 22.1 & 0.01 & 20.99 & 0.01 & 182.0 & 99.0 & 378022.12 & 24251.02 & 0.44 & 0.1 & -1.93 & 1.0\\
  137.580693\_7.035973 & ngc2775 & 137.58069 & 7.03597 & 4308.49 & 3647.61 & 23.36 & 0.16 & 21.64 & 0.03 & 21.26 & 0.01 & 20.43 & 0.01 & 19.09 & 0.01 & 8304.0 & 5049.0 & 9607692.22 & 4436617.95 & 0.0 & 0.06 & -1.86 & 1.0\\
  137.586002\_7.041214 & ngc2775 & 137.586 & 7.04121 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & -1.68 & 1.0\\
  137.607244\_7.041817 & ngc2775 & 137.60724 & 7.04182 & 1914.22 & 4178.8 & 23.77 & 0.23 & 23.45 & 0.14 & 23.21 & 0.03 & 22.42 & 0.02 & 21.36 & 0.01 & 1187.0 & 566.0 & 297932.83 & 46211.3 & 0.07 & 0.2 & -1.63 & 1.0\\
  137.586087\_7.033149 & ngc2775 & 137.58609 & 7.03315 & 3822.06 & 3391.16 & 23.38 & 0.17 & 23.63 & 0.19 & 23.3 & 0.05 & 22.77 & 0.03 & 21.84 & 0.03 & 226.0 & 98.0 & 155184.38 & 28532.53 & 0.33 & 0.14 & -1.76 & 1.0\\
  137.600392\_7.030389 & ngc2775 & 137.60039 & 7.03039 & 2532.04 & 3140.07 & 23.85 & 0.25 & 23.57 & 0.15 & 23.72 & 0.05 & 23.06 & 0.03 & 21.99 & 0.02 & 5.0 & 164.0 & 38131.38 & 91349.01 & 0.89 & 0.48 & -1.67 & 1.0\\
  137.594406\_7.059938 & ngc2775 & 137.59441 & 7.05994 & 3072.04 & 5825.19 & 23.2 & 0.14 & 22.21 & 0.05 & 22.25 & 0.02 & 21.57 & 0.01 & 20.53 & 0.01 & 1276.0 & 248.0 & 646558.51 & 34405.11 & 0.0 & 0.05 & -1.52 & 1.0\\
  137.574894\_7.028595 & ngc2775 & 137.57489 & 7.0286 & 4831.34 & 2977.31 & 24.71 & 0.53 & 23.21 & 0.11 & 22.47 & 0.02 & 21.41 & 0.01 & 19.88 & 0.01 & 956.0 & 7969.0 & 2661887.83 & 5059873.2 & 0.53 & 0.3 & -1.6 & 1.0\\
  137.581066\_7.051743 & ngc2775 & 137.58107 & 7.05174 & 4275.02 & 5080.46 & 20.89 & 0.03 & 21.29 & 0.03 & 22.61 & 0.03 & 22.61 & 0.02 & 22.45 & 0.04 & 1.0 & 5.0 & 25128.95 & 20453.99 & 0.29 & 0.26 & -1.8 & 2.0\\
  137.574292\_7.053071 & ngc2775 & 137.57429 & 7.05307 & 4885.97 & 5201.52 & 20.99 & 0.02 & 21.4 & 0.03 & 22.76 & 0.03 & 22.82 & 0.02 & 22.84 & 0.05 & 3.0 & 2.0 & 11084.47 & 3693.42 & 0.22 & 0.02 & -1.73 & 2.0\\
  137.584837\_7.047262 & ngc2775 & 137.58484 & 7.04726 & 3934.28 & 4673.81 & 20.15 & 0.01 & 20.65 & 0.02 & 22.05 & 0.02 & 22.09 & 0.02 & 22.1 & 0.04 & 1.0 & 2.0 & 30949.36 & 13553.0 & 0.21 & 0.05 & -1.77 & 2.0\\
  137.594515\_7.036721 & ngc2775 & 137.59452 & 7.03672 & 3061.89 & 3715.57 & 18.72 & 0.01 & 19.29 & 0.01 & 20.57 & 0.01 & 20.65 & 0.01 & 20.5 & 0.01 & 6.0 & 3.0 & 26847.83 & 71955.47 & 0.0 & 0.26 & -1.45 & 2.0\\
  137.590265\_7.033135 & ngc2775 & 137.59026 & 7.03314 & 3445.17 & 3389.96 & 20.26 & 0.02 & 20.72 & 0.02 & 22.2 & 0.02 & 22.27 & 0.02 & 22.24 & 0.04 & 1.0 & 0.0 & 25365.96 & 4325.29 & 0.19 & 0.04 & -1.68 & 2.0\\
  137.593421\_7.042283 & ngc2775 & 137.59342 & 7.04228 & 3160.62 & 4220.94 & 19.18 & 0.01 & 19.64 & 0.01 & 20.97 & 0.01 & 21.03 & 0.01 & 20.88 & 0.01 & 1.0 & 3.0 & 100492.9 & 70779.58 & 0.26 & 0.1 & -1.68 & 2.0\\
  137.573564\_7.039912 & ngc2775 & 137.57356 & 7.03991 & 4951.27 & 4005.49 & 21.27 & 0.03 & 21.71 & 0.03 & 23.1 & 0.04 & 23.07 & 0.03 & 22.8 & 0.06 & 1.0 & 0.0 & 16234.25 & 2503.77 & 0.28 & 0.04 & -1.74 & 2.0\\
  137.593695\_7.021097 & ngc2775 & 137.5937 & 7.0211 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & -0.97 & 3.0\\
  137.593373\_7.032235 & ngc2775 & 137.59337 & 7.03224 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & -0.81 & 3.0\\
  137.578326\_7.030815 & ngc2775 & 137.57833 & 7.03082 & 4522.21 & 3179.38 & 20.54 & 0.03 & 20.95 & 0.03 & 22.27 & 0.03 & 22.25 & 0.03 & 22.06 & 0.05 & 1.0 & 3.0 & 36088.42 & 25423.4 & 0.3 & 0.1 & -1.09 & 3.0\\
  137.572681\_7.036065 & ngc2775 & 137.57268 & 7.03606 & 5032.0 & 3655.92 & 20.24 & 0.02 & 20.82 & 0.02 & 22.3 & 0.02 & 22.49 & 0.02 & 22.47 & 0.05 & 1.0 & 3.0 & 17824.22 & 12973.54 & 0.13 & 0.12 & -1.14 & 3.0\\
  137.574311\_7.048193 & ngc2775 & 137.57431 & 7.04819 & 4884.28 & 4757.97 & 21.01 & 0.03 & 21.37 & 0.03 & 22.81 & 0.03 & 22.85 & 0.03 & 22.5 & 0.05 & 1.0 & 2.0 & 20977.02 & 9211.03 & 0.28 & 0.05 & -1.74 & 3.0\\
  137.573513\_7.047533 & ngc2775 & 137.57351 & 7.04753 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & -0.88 & 3.0\\
  137.581064\_7.0486 & ngc2775 & 137.58106 & 7.0486 & 4275.13 & 4795.1 & 22.01 & 0.06 & 22.02 & 0.06 & 22.5 & 0.03 & 22.37 & 0.02 & 21.98 & 0.04 & 136.0 & 34.0 & 62858.32 & 1182.42 & 0.0 & 0.06 & -1.65 & 3.0\\
  137.58947\_7.047775 & ngc2775 & 137.58947 & 7.04778 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & -0.82 & 3.0\\
  137.577161\_7.032015 & ngc2775 & 137.57716 & 7.03202 & 4626.34 & 3288.63 & 22.56 & 0.09 & 22.69 & 0.09 & 22.94 & 0.03 & 22.42 & 0.02 & 21.69 & 0.03 & 95.0 & 7.0 & 107530.86 & 11955.34 & 0.28 & 0.05 & -1.21 & 3.0\\
  137.575919\_7.03371 & ngc2775 & 137.57592 & 7.03371 & 4739.27 & 3442.93 & 21.58 & 0.04 & 21.67 & 0.04 & 22.32 & 0.02 & 21.93 & 0.02 & 21.25 & 0.02 & 6.0 & 70.0 & 29045.86 & 74369.33 & 0.45 & 0.31 & -1.57 & 3.0\\
  139.452634\_-22.342288 & ngc2835 & 139.45263 & -22.34229 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & -1.45 & 1.0\\
  139.486041\_-22.348162 & ngc2835 & 139.48604 & -22.34816 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & -1.63 & 1.0\\
  139.483405\_-22.347063 & ngc2835 & 139.4834 & -22.34706 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & -1.59 & 1.0\\
  139.454426\_-22.365589 & ngc2835 & 139.45443 & -22.36559 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & -1.65 & 1.0\\
  139.485389\_-22.375795 & ngc2835 & 139.48539 & -22.3758 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & -1.51 & 1.0\\
  139.466657\_-22.372925 & ngc2835 & 139.46666 & -22.37292 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & -1.49 & 1.0\\
  139.473233\_-22.371925 & ngc2835 & 139.47323 & -22.37192 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & -1.65 & 1.0\\
  139.486403\_-22.365206 & ngc2835 & 139.4864 & -22.36521 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & -1.72 & 1.0\\
  139.46781\_-22.35852 & ngc2835 & 139.46781 & -22.35852 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & -1.8 & 1.0\\
  139.461431\_-22.36684 & ngc2835 & 139.46143 & -22.36684 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & -1.69 & 1.0\\
  139.461841\_-22.336557 & ngc2835 & 139.46184 & -22.33656 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & -1.64 & 2.0\\
  139.469967\_-22.335052 & ngc2835 & 139.46997 & -22.33505 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & -1.71 & 2.0\\
  139.474737\_-22.350525 & ngc2835 & 139.47474 & -22.35052 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & -1.7 & 2.0\\
  139.455839\_-22.337762 & ngc2835 & 139.45584 & -22.33776 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & -1.61 & 2.0\\
  139.454881\_-22.342227 & ngc2835 & 139.45488 & -22.34223 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & -0.95 & 2.0\\
  139.459764\_-22.370211 & ngc2835 & 139.45976 & -22.37021 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & -1.66 & 2.0\\
  139.471387\_-22.366178 & ngc2835 & 139.47139 & -22.36618 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & -1.66 & 2.0\\
  139.490274\_-22.363176 & ngc2835 & 139.49027 & -22.36318 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & -1.64 & 2.0\\
  139.47114\_-22.370214 & ngc2835 & 139.47114 & -22.37021 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & -1.26 & 2.0\\
  139.447406\_-22.35416 & ngc2835 & 139.44741 & -22.35416 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & -1.46 & 2.0\\
  139.486032\_-22.356806 & ngc2835 & 139.48603 & -22.35681 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & -1.67 & 2.0\\
  139.469144\_-22.336093 & ngc2835 & 139.46914 & -22.33609 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & -0.86 & 3.0\\
  139.457309\_-22.331832 & ngc2835 & 139.45731 & -22.33183 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & -1.19 & 3.0\\
  139.467765\_-22.336642 & ngc2835 & 139.46776 & -22.33664 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & -1.66 & 3.0\\
  139.484821\_-22.358857 & ngc2835 & 139.48482 & -22.35886 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & -1.48 & 3.0\\
  139.475553\_-22.359698 & ngc2835 & 139.47555 & -22.3597 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & -1.87 & 3.0\\
  139.452335\_-22.34128 & ngc2835 & 139.45234 & -22.34128 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & -1.68 & 3.0\\
  139.462585\_-22.336393 & ngc2835 & 139.46259 & -22.33639 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & -0.7 & 3.0\\
  139.455409\_-22.337422 & ngc2835 & 139.45541 & -22.33742 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & -1.85 & 3.0\\
  139.458125\_-22.360977 & ngc2835 & 139.45812 & -22.36098 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & -0.8 & 3.0\\
  160.973027\_11.708071 & ngc3351 & 160.97303 & 11.70807 & 7706.42 & 6881.28 & 22.92 & 0.09 & 22.59 & 0.05 & 22.59 & 0.02 & 22.03 & 0.01 & 20.94 & 0.01 & 127.0 & 9.0 & 62565.13 & 8978.5 & 0.46 & 0.03 & -1.71 & 1.0\\
  160.990601\_11.696827 & ngc3351 & 160.9906 & 11.69683 & 6142.83 & 5859.69 & 23.54 & 0.15 & 22.79 & 0.07 & 22.54 & 0.02 & 21.93 & 0.01 & 20.72 & 0.01 & 210.0 & 16.0 & 110747.6 & 14943.74 & 0.52 & 0.03 & -1.82 & 1.0\\
  161.006225\_11.714776 & ngc3351 & 161.00622 & 11.71478 & 4753.07 & 7490.66 & 20.6 & 0.02 & 20.72 & 0.02 & 21.36 & 0.01 & 21.21 & 0.01 & 20.56 & 0.01 & 71.0 & 18.0 & 34749.64 & 363.6 & 0.1 & 0.06 & -1.71 & 1.0\\
  160.995868\_11.705519 & ngc3351 & 160.99587 & 11.70552 & 5674.3 & 6649.39 & 23.33 & 0.12 & 22.53 & 0.05 & 22.56 & 0.02 & 21.97 & 0.01 & 20.83 & 0.01 & 158.0 & 52.0 & 79163.82 & 17367.07 & 0.48 & 0.0 & -1.63 & 1.0\\
  160.980705\_11.702128 & ngc3351 & 160.9807 & 11.70213 & 7023.46 & 6341.32 & 24.93 & 0.55 & 25.71 & 0.91 & 23.86 & 0.06 & 23.13 & 0.02 & 21.85 & 0.02 & 465.0 & 222.0 & 55498.87 & 10894.34 & 0.5 & 0.08 & -1.73 & 1.0\\
  160.993362\_11.713569 & ngc3351 & 160.99336 & 11.71357 & 5897.37 & 7380.96 & 25.01 & 0.52 & 22.96 & 0.08 & 22.58 & 0.02 & 21.77 & 0.01 & 20.4 & 0.01 & 6690.0 & 3871.0 & 485917.35 & 131926.87 & 0.03 & 0.14 & -1.69 & 1.0\\
  160.993486\_11.682149 & ngc3351 & 160.99349 & 11.68215 & 5886.18 & 4525.98 & 23.88 & 0.18 & 24.13 & 0.2 & 23.76 & 0.05 & 23.6 & 0.02 & 23.01 & 0.04 & 324.0 & 114.0 & 6319.24 & 1111.14 & 0.0 & 0.14 & -1.73 & 1.0\\
  160.993972\_11.690572 & ngc3351 & 160.99397 & 11.69057 & 5842.76 & 5291.51 & 24.07 & 0.23 & 23.09 & 0.08 & 23.13 & 0.03 & 22.39 & 0.01 & 21.08 & 0.01 & 110.0 & 39.0 & 73347.08 & 10125.04 & 0.65 & 0.04 & -1.61 & 1.0\\
  160.987016\_11.709356 & ngc3351 & 160.98702 & 11.70936 & 6461.89 & 6998.26 & 23.32 & 0.12 & 22.68 & 0.06 & 22.62 & 0.02 & 22.06 & 0.01 & 20.95 & 0.01 & 169.0 & 22.0 & 71911.48 & 11238.49 & 0.46 & 0.02 & -1.77 & 1.0\\
  160.994709\_11.719698 & ngc3351 & 160.99471 & 11.7197 & 5777.64 & 7937.9 & 21.08 & 0.03 & 21.22 & 0.03 & 21.93 & 0.02 & 21.95 & 0.01 & 21.56 & 0.02 & 5.0 & 0.0 & 4054.54 & 474.68 & 0.34 & 0.03 & -1.83 & 1.0\\
  160.975029\_11.711627 & ngc3351 & 160.97503 & 11.71163 & 7528.71 & 7203.88 & 22.71 & 0.07 & 22.63 & 0.06 & 23.22 & 0.03 & 23.02 & 0.02 & 22.35 & 0.03 & 88.0 & 35.0 & 7869.99 & 692.76 & 0.13 & 0.07 & -1.5 & 2.0\\
  160.960895\_11.680389 & ngc3351 & 160.9609 & 11.68039 & 8785.88 & 4365.48 & 17.89 & 0.01 & 18.48 & 0.01 & 20.16 & 0.01 & 20.37 & 0.01 & 20.1 & 0.02 & 1.0 & 2.0 & 24082.9 & 9412.34 & 0.11 & 0.03 & -1.63 & 2.0\\
  161.006971\_11.708431 & ngc3351 & 161.00697 & 11.70843 & 4686.22 & 6914.31 & 18.4 & 0.01 & 18.99 & 0.01 & 20.59 & 0.02 & 20.76 & 0.02 & 20.71 & 0.02 & 1.0 & 1.0 & 15704.92 & 1411.6 & 0.11 & 0.03 & -1.8 & 2.0\\
  160.967076\_11.715766 & ngc3351 & 160.96708 & 11.71577 & 8236.11 & 7580.81 & 19.71 & 0.02 & 20.07 & 0.02 & 21.49 & 0.02 & 21.44 & 0.02 & 21.15 & 0.02 & 1.0 & 0.0 & 15152.93 & 2472.72 & 0.31 & 0.04 & -1.68 & 2.0\\
  160.975645\_11.685276 & ngc3351 & 160.97564 & 11.68528 & 7472.94 & 4810.04 & 23.31 & 0.13 & 23.28 & 0.1 & 23.63 & 0.04 & 23.38 & 0.02 & 22.75 & 0.04 & 136.0 & 11.0 & 6772.16 & 1126.55 & 0.12 & 0.07 & -1.67 & 2.0\\
  161.009113\_11.702444 & ngc3351 & 161.00911 & 11.70244 & 4495.84 & 6369.95 & 19.43 & 0.01 & 19.83 & 0.01 & 20.95 & 0.01 & 20.93 & 0.01 & 20.0 & 0.01 & 9.0 & 2.0 & 10021.35 & 2875.12 & 0.09 & 0.01 & -1.66 & 2.0\\
  161.005048\_11.6898 & ngc3351 & 161.00505 & 11.6898 & 4857.52 & 5221.41 & 21.35 & 0.03 & 21.72 & 0.04 & 22.73 & 0.03 & 22.72 & 0.03 & 22.27 & 0.05 & 7.0 & 0.0 & 1215.04 & 201.71 & 0.12 & 0.04 & -1.56 & 2.0\\
  161.009941\_11.716747 & ngc3351 & 161.00994 & 11.71675 & 4422.34 & 7669.86 & 19.74 & 0.01 & 20.08 & 0.01 & 21.52 & 0.01 & 21.55 & 0.01 & 21.52 & 0.02 & 1.0 & 1.0 & 10492.83 & 946.91 & 0.24 & 0.03 & -1.5 & 2.0\\
  160.975484\_11.686687 & ngc3351 & 160.97548 & 11.68669 & 7488.34 & 4938.81 & 19.66 & 0.01 & 20.12 & 0.01 & 21.58 & 0.01 & 21.7 & 0.01 & 21.67 & 0.02 & 1.0 & 0.0 & 8138.14 & 984.72 & 0.19 & 0.03 & -1.61 & 2.0\\
  160.979312\_11.684669 & ngc3351 & 160.97931 & 11.68467 & 7147.34 & 4754.56 & 22.5 & 0.06 & 22.57 & 0.05 & 23.03 & 0.03 & 22.9 & 0.01 & 22.26 & 0.02 & 102.0 & 7.0 & 8596.47 & 1060.42 & 0.09 & 0.05 & -1.64 & 2.0\\
  160.973571\_11.696571 & ngc3351 & 160.97357 & 11.69657 & 7657.83 & 5836.3 & 24.78 & 0.49 & 23.29 & 0.11 & 23.42 & 0.04 & 22.72 & 0.01 & 21.57 & 0.01 & 1829.0 & 458.0 & 60807.6 & 2151.25 & 0.0 & 0.11 & -1.59 & 2.0\\
  160.972103\_11.715843 & ngc3351 & 160.9721 & 11.71584 & 7788.86 & 7587.64 & 21.4 & 0.04 & 21.76 & 0.04 & 23.25 & 0.04 & 23.32 & 0.04 & 23.46 & 0.09 & 3.0 & 2.0 & 1098.66 & 936.82 & 0.17 & 0.06 & -1.82 & 3.0\\
  160.981298\_11.719904 & ngc3351 & 160.9813 & 11.7199 & 6970.89 & 7956.34 & 19.96 & 0.02 & 20.43 & 0.02 & 21.97 & 0.02 & 22.12 & 0.02 & 22.22 & 0.04 & 1.0 & 3.0 & 4480.92 & 3209.22 & 0.13 & 0.11 & -0.97 & 3.0\\
  160.974944\_11.700948 & ngc3351 & 160.97494 & 11.70095 & 7535.75 & 6233.65 & 22.31 & 0.06 & 22.7 & 0.08 & 23.79 & 0.06 & 23.89 & 0.05 & 23.68 & 0.11 & 6.0 & 3.0 & 293.51 & 974.69 & 0.06 & 0.3 & -0.94 & 3.0\\
  160.971492\_11.706538 & ngc3351 & 160.97149 & 11.70654 & 7842.95 & 6742.01 & 19.68 & 0.01 & 20.03 & 0.01 & 21.7 & 0.02 & 21.66 & 0.01 & 21.37 & 0.02 & 1.0 & 2.0 & 10239.96 & 3996.94 & 0.24 & 0.03 & -0.79 & 3.0\\
  160.985228\_11.68858 & ngc3351 & 160.98523 & 11.68858 & 6621.05 & 5110.19 & 20.61 & 0.02 & 20.42 & 0.01 & 21.67 & 0.01 & 21.87 & 0.01 & 21.32 & 0.02 & 1.0 & 0.0 & 17435.21 & 2071.55 & 0.45 & 0.03 & -0.82 & 3.0\\
  160.992406\_11.685644 & ngc3351 & 160.99241 & 11.68564 & 5982.35 & 4842.69 & 19.38 & 0.02 & 19.94 & 0.02 & 21.6 & 0.02 & 21.88 & 0.02 & 21.87 & 0.03 & 1.0 & 0.0 & 4922.83 & 828.19 & 0.06 & 0.04 & -1.68 & 3.0\\
  160.996282\_11.688622 & ngc3351 & 160.99628 & 11.68862 & 5637.18 & 5114.35 & 20.7 & 0.04 & 21.34 & 0.04 & 22.73 & 0.04 & 23.0 & 0.05 & 22.97 & 0.09 & 4.0 & 3.0 & 552.23 & 1937.65 & 0.0 & 0.17 & -1.03 & 3.0\\
  160.978131\_11.691236 & ngc3351 & 160.97813 & 11.69124 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & -0.96 & 3.0\\
  161.001552\_11.695959 & ngc3351 & 161.00155 & 11.69596 & 5168.37 & 5781.52 & 19.77 & 0.01 & 20.26 & 0.01 & 21.78 & 0.01 & 21.88 & 0.01 & 21.91 & 0.03 & 1.0 & 2.0 & 6172.08 & 2698.83 & 0.16 & 0.05 & -1.76 & 3.0\\
  160.978158\_11.691254 & ngc3351 & 160.97816 & 11.69125 & 7250.84 & 5353.82 & 20.58 & 0.02 & 21.12 & 0.03 & 22.65 & 0.04 & 22.73 & 0.02 & 22.67 & 0.04 & 1.0 & 0.0 & 2976.4 & 449.19 & 0.17 & 0.04 & -0.64 & 3.0\\
  160.991619\_11.70277 & ngc3351 & 160.99162 & 11.70277 & 6052.45 & 6399.74 & 16.88 & 0.01 & 17.22 & 0.01 & 18.39 & 0.01 & 18.43 & 0.01 & 17.87 & 0.02 & 8.0 & 0.0 & 67225.08 & 7589.6 & 0.06 & 0.03 & -1.75 & 1.0\\
  160.991797\_11.703236 & ngc3351 & 160.9918 & 11.70324 & 6036.49 & 6442.11 & 17.32 & 0.01 & 17.66 & 0.01 & 18.87 & 0.02 & 18.9 & 0.02 & 18.22 & 0.01 & 8.0 & 0.0 & 46762.61 & 5260.16 & 0.07 & 0.03 & -1.79 & 1.0\\
  170.058865\_12.984064 & ngc3627 & 170.05886 & 12.98406 & 7258.68 & 7282.78 & 20.28 & 0.01 & 20.14 & 0.01 & 20.24 & 0.01 & 20.06 & 0.01 & 19.36 & 0.01 & 196.0 & 47.0 & 246013.34 & 48550.87 & 0.13 & 0.1 & -1.72 & 1.0\\
  170.054868\_13.018927 & ngc3627 & 170.05487 & 13.01893 & 7612.68 & 10450.41 & 23.35 & 0.19 & 22.61 & 0.09 & 22.49 & 0.03 & 22.08 & 0.02 & 21.22 & 0.02 & 770.0 & 544.0 & 64918.76 & 1184.41 & 0.0 & 0.31 & -1.52 & 1.0\\
  170.05244\_12.997817 & ngc3627 & 170.05244 & 12.99782 & 7827.18 & 8531.78 & 19.8 & 0.02 & 19.69 & 0.01 & 20.18 & 0.01 & 19.98 & 0.01 & 19.18 & 0.01 & 88.0 & 7.0 & 205496.59 & 28586.34 & 0.19 & 0.02 & -1.7 & 1.0\\
  170.059425\_12.98024 & ngc3627 & 170.05942 & 12.98024 & 7209.05 & 6935.23 & 20.24 & 0.01 & 20.48 & 0.01 & 21.3 & 0.01 & 21.27 & 0.01 & 20.77 & 0.02 & 53.0 & 46.0 & 26216.27 & 18622.1 & 0.0 & 0.21 & -1.79 & 1.0\\
  170.067557\_13.001399 & ngc3627 & 170.06756 & 13.0014 & 6489.1 & 8857.81 & 19.58 & 0.01 & 19.71 & 0.01 & 20.24 & 0.01 & 20.21 & 0.01 & 19.7 & 0.01 & 110.0 & 28.0 & 109629.49 & 15427.27 & 0.01 & 0.02 & -1.77 & 1.0\\
  170.061027\_12.974435 & ngc3627 & 170.06103 & 12.97444 & 7067.32 & 6407.69 & 18.6 & 0.01 & 18.9 & 0.01 & 19.75 & 0.01 & 19.68 & 0.01 & 18.92 & 0.01 & 32.0 & 14.0 & 120732.49 & 5458.69 & 0.1 & 0.05 & -1.65 & 1.0\\
  170.053112\_12.999744 & ngc3627 & 170.05311 & 12.99974 & 7767.91 & 8707.53 & 20.52 & 0.02 & 20.5 & 0.02 & 20.95 & 0.01 & 20.81 & 0.01 & 20.08 & 0.02 & 95.0 & 32.0 & 85508.56 & 12919.78 & 0.14 & 0.02 & -1.63 & 1.0\\
  170.056703\_12.995196 & ngc3627 & 170.0567 & 12.9952 & 7450.03 & 8294.19 & 19.88 & 0.02 & 19.53 & 0.01 & 19.41 & 0.01 & 19.18 & 0.0 & 18.47 & 0.01 & 375.0 & 51.0 & 619319.71 & 46724.33 & 0.04 & 0.06 & -1.71 & 1.0\\
  170.044676\_13.008662 & ngc3627 & 170.04468 & 13.00866 & 8514.35 & 9517.36 & 22.26 & 0.09 & 21.94 & 0.05 & 21.75 & 0.02 & 21.49 & 0.01 & 20.85 & 0.02 & 403.0 & 122.0 & 72985.03 & 4268.66 & 0.03 & 0.08 & -1.62 & 1.0\\
  170.051696\_12.999426 & ngc3627 & 170.0517 & 12.99943 & 7893.43 & 8678.67 & 20.84 & 0.03 & 20.63 & 0.02 & 20.98 & 0.01 & 20.66 & 0.01 & 19.8 & 0.01 & 102.0 & 14.0 & 148082.33 & 10516.02 & 0.27 & 0.05 & -1.76 & 1.0\\
  170.068223\_12.998414 & ngc3627 & 170.06822 & 12.99841 & 6430.08 & 8586.8 & 17.61 & 0.01 & 17.93 & 0.01 & 18.97 & 0.01 & 18.95 & 0.0 & 18.3 & 0.01 & 8.0 & 14.0 & 65364.24 & 83679.41 & 0.13 & 0.09 & -1.67 & 2.0\\
  170.074936\_12.985122 & ngc3627 & 170.07494 & 12.98512 & 5835.89 & 7378.77 & 17.36 & 0.0 & 17.67 & 0.0 & 18.74 & 0.0 & 18.63 & 0.0 & 18.1 & 0.0 & 7.0 & 21.0 & 76196.13 & 125865.88 & 0.16 & 0.15 & -1.61 & 2.0\\
  170.069672\_12.992535 & ngc3627 & 170.06967 & 12.99254 & 6301.62 & 8052.81 & 18.45 & 0.01 & 18.73 & 0.01 & 19.7 & 0.01 & 19.67 & 0.01 & 19.01 & 0.01 & 32.0 & 25.0 & 100963.73 & 63329.62 & 0.04 & 0.18 & -1.76 & 2.0\\
  170.071929\_12.974778 & ngc3627 & 170.07193 & 12.97478 & 6102.05 & 6439.07 & 17.67 & 0.01 & 17.96 & 0.01 & 18.9 & 0.01 & 18.87 & 0.01 & 18.09 & 0.01 & 30.0 & 6.0 & 217672.29 & 37053.89 & 0.06 & 0.0 & -1.66 & 2.0\\
  170.052507\_12.967423 & ngc3627 & 170.05251 & 12.96742 & 7821.67 & 5770.95 & 19.68 & 0.01 & 19.64 & 0.01 & 19.7 & 0.01 & 19.61 & 0.01 & 19.01 & 0.01 & 243.0 & 33.0 & 286407.11 & 60268.54 & 0.01 & 0.08 & -1.67 & 2.0\\
  170.066268\_12.97554 & ngc3627 & 170.06627 & 12.97554 & 6603.17 & 6508.32 & 18.97 & 0.01 & 19.13 & 0.01 & 19.91 & 0.01 & 19.8 & 0.01 & 18.86 & 0.01 & 30.0 & 17.0 & 132776.43 & 63047.47 & 0.18 & 0.04 & -1.64 & 2.0\\
  170.074834\_12.981697 & ngc3627 & 170.07483 & 12.9817 & 5844.83 & 7067.73 & 20.71 & 0.02 & 20.5 & 0.02 & 20.83 & 0.01 & 20.42 & 0.01 & 19.16 & 0.01 & 46.0 & 20.0 & 219460.49 & 20344.18 & 0.47 & 0.05 & -1.61 & 2.0\\
  170.053916\_12.988423 & ngc3627 & 170.05392 & 12.98842 & 7697.1 & 7678.18 & 19.63 & 0.01 & 19.6 & 0.01 & 19.91 & 0.01 & 19.79 & 0.01 & 19.22 & 0.01 & 169.0 & 51.0 & 209918.69 & 22599.36 & 0.03 & 0.1 & -1.71 & 2.0\\
  170.059237\_12.983306 & ngc3627 & 170.05924 & 12.98331 & 7225.88 & 7213.99 & 20.01 & 0.02 & 19.97 & 0.01 & 20.58 & 0.01 & 20.33 & 0.01 & 19.31 & 0.01 & 40.0 & 6.0 & 128988.28 & 19566.25 & 0.29 & 0.01 & -1.71 & 2.0\\
  170.07467\_13.010645 & ngc3627 & 170.07467 & 13.01064 & 5859.27 & 9697.72 & 21.32 & 0.07 & 21.06 & 0.04 & 22.13 & 0.06 & 21.94 & 0.06 & 21.53 & 0.05 & 3.0 & 1.0 & 16437.72 & 7883.52 & 0.56 & 0.05 & -0.85 & 3.0\\
  170.051309\_13.004617 & ngc3627 & 170.05131 & 13.00462 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & -0.96 & 3.0\\
  170.047688\_12.988798 & ngc3627 & 170.04769 & 12.9888 & 8248.04 & 7712.93 & 22.39 & 0.11 & 22.46 & 0.08 & 23.4 & 0.06 & 23.33 & 0.06 & 22.27 & 0.06 & 21.0 & 9.0 & 4590.67 & 1497.56 & 0.2 & 0.01 & -0.87 & 3.0\\
  170.066031\_12.973518 & ngc3627 & 170.06603 & 12.97352 & 6624.0 & 6324.57 & 22.09 & 0.1 & 22.59 & 0.15 & 23.5 & 0.11 & 23.39 & 0.08 & 23.02 & 0.12 & 7.0 & 1.0 & 846.54 & 195.66 & 0.14 & 0.1 & -0.61 & 3.0\\
  170.049066\_12.977681 & ngc3627 & 170.04907 & 12.97768 & 8125.98 & 6703.3 & 21.57 & 0.03 & 21.36 & 0.03 & 22.19 & 0.03 & 21.76 & 0.03 & 20.76 & 0.02 & 7.0 & 6.0 & 11977.12 & 49572.57 & 0.5 & 0.29 & -1.58 & 3.0\\
  170.048767\_12.98418 & ngc3627 & 170.04877 & 12.98418 & 8152.83 & 7294.11 & 20.59 & 0.03 & 20.58 & 0.03 & 21.41 & 0.02 & 21.11 & 0.02 & 20.37 & 0.02 & 7.0 & 5.0 & 14654.21 & 48696.14 & 0.38 & 0.3 & -1.64 & 3.0\\
  170.067815\_13.00359 & ngc3627 & 170.06782 & 13.00359 & 6466.68 & 9056.79 & 19.41 & 0.02 & 19.83 & 0.02 & 21.02 & 0.02 & 21.09 & 0.02 & 20.61 & 0.03 & 8.0 & 1.0 & 6269.23 & 39.63 & 0.01 & 0.05 & -1.31 & 3.0\\
  170.068235\_13.001602 & ngc3627 & 170.06824 & 13.0016 & 6429.42 & 8876.45 & 18.86 & 0.03 & 19.31 & 0.03 & 20.74 & 0.03 & 20.84 & 0.03 & 20.75 & 0.04 & 1.0 & 0.0 & 24539.39 & 4150.98 & 0.21 & 0.04 & -0.7 & 3.0\\
  170.048899\_12.988845 & ngc3627 & 170.0489 & 12.98884 & 8141.89 & 7717.07 & 20.73 & 0.06 & 20.84 & 0.05 & 21.67 & 0.03 & 21.28 & 0.02 & 20.39 & 0.02 & 8.0 & 16.0 & 14652.14 & 15048.0 & 0.37 & 0.14 & -1.55 & 3.0\\
  188.580776\_8.196998 & ngc4535 & 188.58078 & 8.197 & 3776.89 & 3100.86 & 24.91 & 0.75 & 23.76 & 0.23 & 23.5 & 0.05 & 22.93 & 0.03 & 21.76 & 0.03 & 281.0 & 995.0 & 93827.25 & 29708.03 & 0.42 & 0.3 & -1.87 & 1.0\\
  188.581583\_8.196693 & ngc4535 & 188.58158 & 8.19669 & 3704.31 & 3073.24 & 24.7 & 0.6 & 23.97 & 0.28 & 24.03 & 0.08 & 23.33 & 0.05 & 22.16 & 0.04 & 5.0 & 1023.0 & 16988.89 & 78071.81 & 0.96 & 0.72 & -1.8 & 1.0\\
  188.583789\_8.180033 & ngc4535 & 188.58379 & 8.18003 & 3505.85 & 1559.33 & 20.83 & 0.02 & 20.92 & 0.02 & 21.5 & 0.01 & 21.43 & 0.01 & 20.92 & 0.01 & 110.0 & 17.0 & 68367.47 & 6917.86 & 0.01 & 0.0 & -1.73 & 1.0\\
  188.603201\_8.200501 & ngc4535 & 188.6032 & 8.2005 & 1759.96 & 3419.0 & 18.41 & 0.01 & 18.85 & 0.01 & 20.3 & 0.01 & 20.62 & 0.01 & 20.28 & 0.01 & 1.0 & 2.0 & 63012.95 & 26072.18 & 0.19 & 0.04 & -1.4 & 1.0\\
  188.566124\_8.206946 & ngc4535 & 188.56612 & 8.20695 & 5094.56 & 4004.97 & 22.7 & 0.1 & 22.02 & 0.05 & 22.1 & 0.02 & 21.49 & 0.01 & 20.4 & 0.01 & 136.0 & 74.0 & 275545.77 & 21240.02 & 0.48 & 0.07 & -1.55 & 1.0\\
  188.562963\_8.214193 & ngc4535 & 188.56296 & 8.21419 & 5379.06 & 4663.35 & 23.31 & 0.17 & 23.13 & 0.11 & 23.4 & 0.05 & 23.21 & 0.03 & 22.52 & 0.04 & 158.0 & 70.0 & 21980.07 & 1706.84 & 0.12 & 0.09 & -1.46 & 1.0\\
  188.582003\_8.195665 & ngc4535 & 188.582 & 8.19566 & 3666.36 & 2979.72 & 24.93 & 0.75 & 23.67 & 0.21 & 23.7 & 0.07 & 23.02 & 0.03 & 21.76 & 0.03 & 147.0 & 45.0 & 93282.0 & 10366.83 & 0.57 & 0.11 & -1.64 & 1.0\\
  188.573243\_8.180181 & ngc4535 & 188.57324 & 8.18018 & 4453.94 & 1573.2 & 22.69 & 0.1 & 22.65 & 0.08 & 22.75 & 0.03 & 22.66 & 0.02 & 22.15 & 0.03 & 226.0 & 44.0 & 30755.82 & 2128.08 & 0.0 & 0.02 & -1.6 & 1.0\\
  188.582318\_8.180233 & ngc4535 & 188.58232 & 8.18023 & 3638.25 & 1577.65 & 21.37 & 0.04 & 21.52 & 0.03 & 22.05 & 0.02 & 21.95 & 0.01 & 21.37 & 0.02 & 95.0 & 34.0 & 43335.08 & 2501.4 & 0.05 & 0.07 & -1.65 & 1.0\\
  188.567824\_8.185806 & ngc4535 & 188.56782 & 8.18581 & 4941.47 & 2084.16 & 23.28 & 0.17 & 23.16 & 0.12 & 22.87 & 0.03 & 22.66 & 0.02 & 22.07 & 0.03 & 403.0 & 54.0 & 44116.96 & 4031.86 & 0.0 & 0.07 & -1.68 & 1.0\\
  188.585754\_8.185512 & ngc4535 & 188.58575 & 8.18551 & 3329.07 & 2057.3 & 24.24 & 0.4 & 22.57 & 0.07 & 22.4 & 0.02 & 21.61 & 0.01 & 20.29 & 0.01 & 2440.0 & 379.0 & 715243.45 & 93022.61 & 0.08 & 0.08 & -1.63 & 1.0\\
  188.5856\_8.194235 & ngc4535 & 188.5856 & 8.19424 & 3342.85 & 2850.06 & 24.62 & 0.58 & 22.83 & 0.11 & 23.13 & 0.04 & 22.1 & 0.02 & 20.52 & 0.01 & 3.0 & 0.0 & 325065.5 & 52068.18 & 1.39 & 0.06 & -1.71 & 1.0\\
  188.589537\_8.220582 & ngc4535 & 188.58954 & 8.22058 & 2989.16 & 5243.94 & 19.43 & 0.01 & 19.97 & 0.02 & 21.41 & 0.02 & 21.45 & 0.02 & 20.66 & 0.02 & 9.0 & 1.0 & 12538.5 & 2230.93 & 0.0 & 0.0 & -1.77 & 2.0\\
  188.598306\_8.224179 & ngc4535 & 188.59831 & 8.22418 & 2200.18 & 5570.91 & 23.26 & 0.15 & 23.52 & 0.17 & 23.7 & 0.06 & 23.75 & 0.06 & 23.3 & 0.09 & 136.0 & 18.0 & 8645.37 & 1773.67 & 0.0 & 0.08 & -1.73 & 2.0\\
  188.570624\_8.20803 & ngc4535 & 188.57062 & 8.20803 & 4689.77 & 4103.66 & 19.01 & 0.01 & 19.28 & 0.01 & 20.58 & 0.01 & 20.46 & 0.01 & 20.01 & 0.01 & 8.0 & 7.0 & 23924.55 & 113551.53 & 0.06 & 0.37 & -1.76 & 2.0\\
  188.601477\_8.218757 & ngc4535 & 188.60148 & 8.21876 & 1915.2 & 5077.95 & 20.84 & 0.02 & 20.83 & 0.02 & 20.89 & 0.01 & 20.78 & 0.01 & 20.26 & 0.01 & 243.0 & 61.0 & 178461.79 & 22257.01 & 0.0 & 0.09 & -1.73 & 2.0\\
  188.5705\_8.175905 & ngc4535 & 188.5705 & 8.1759 & 4701.07 & 1184.74 & 18.7 & 0.01 & 19.08 & 0.01 & 20.5 & 0.01 & 20.54 & 0.01 & 20.23 & 0.01 & 1.0 & 1.0 & 84480.46 & 25967.85 & 0.29 & 0.04 & -1.67 & 2.0\\
  188.591509\_8.179949 & ngc4535 & 188.59151 & 8.17995 & 2811.4 & 1551.81 & 17.79 & 0.01 & 18.26 & 0.01 & 19.62 & 0.01 & 19.69 & 0.01 & 19.58 & 0.01 & 1.0 & 1.0 & 149227.34 & 13554.94 & 0.24 & 0.03 & -1.62 & 2.0\\
  188.56618\_8.197424 & ngc4535 & 188.56618 & 8.19742 & 5089.65 & 3139.66 & 18.6 & 0.01 & 19.01 & 0.01 & 20.47 & 0.01 & 20.5 & 0.01 & 20.27 & 0.01 & 1.0 & 2.0 & 78369.83 & 24639.96 & 0.26 & 0.0 & -1.64 & 2.0\\
  188.580178\_8.199211 & ngc4535 & 188.58018 & 8.19921 & 3831.22 & 3301.56 & 26.63 & 3.51 & 24.03 & 0.28 & 23.71 & 0.07 & 23.36 & 0.04 & 22.48 & 0.05 & 621.0 & 340.0 & 41092.33 & 1670.33 & 0.08 & 0.22 & -1.72 & 2.0\\
  188.604062\_8.199804 & ngc4535 & 188.60406 & 8.1998 & 1682.57 & 3355.81 & 23.24 & 0.16 & 23.08 & 0.12 & 23.31 & 0.05 & 23.22 & 0.04 & 22.89 & 0.07 & 196.0 & 14.0 & 16471.42 & 2364.79 & 0.0 & 0.03 & -1.71 & 2.0\\
  188.595217\_8.181166 & ngc4535 & 188.59522 & 8.18117 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & -1.47 & 2.0\\
  188.578743\_8.21747 & ngc4535 & 188.57874 & 8.21747 & 3959.77 & 4960.91 & 22.42 & 0.13 & 22.52 & 0.11 & 23.78 & 0.09 & 23.92 & 0.13 & 23.33 & 0.13 & 1.0 & 3.0 & 5717.73 & 3693.98 & 0.4 & 0.05 & -0.65 & 3.0\\
  188.568193\_8.190355 & ngc4535 & 188.56819 & 8.19036 & 4909.52 & 2497.49 & 21.69 & 0.06 & 21.73 & 0.05 & 22.93 & 0.05 & 22.72 & 0.04 & 22.34 & 0.07 & 1.0 & 2.0 & 18910.78 & 4390.1 & 0.49 & 0.03 & -0.85 & 3.0\\
  188.59653\_8.188131 & ngc4535 & 188.59653 & 8.18813 & 2359.94 & 2294.9 & 19.39 & 0.04 & 19.84 & 0.04 & 21.32 & 0.04 & 21.42 & 0.04 & 21.22 & 0.04 & 1.0 & 0.0 & 30088.64 & 4413.7 & 0.22 & 0.04 & -1.18 & 3.0\\
  188.572845\_8.211563 & ngc4535 & 188.57284 & 8.21156 & 4489.34 & 4424.7 & 19.84 & 0.03 & 20.39 & 0.03 & 21.82 & 0.03 & 21.8 & 0.03 & 21.55 & 0.04 & 1.0 & 6.0 & 22263.44 & 17210.5 & 0.25 & 0.25 & -0.97 & 3.0\\
  188.563196\_8.212986 & ngc4535 & 188.5632 & 8.21299 & 5357.87 & 4553.45 & 20.63 & 0.02 & 21.1 & 0.03 & 22.65 & 0.03 & 22.75 & 0.03 & 22.62 & 0.05 & 1.0 & 1.0 & 7649.36 & 652.46 & 0.18 & 0.03 & -0.86 & 3.0\\
  188.570358\_8.176059 & ngc4535 & 188.57036 & 8.17606 & 4713.84 & 1198.22 & 20.91 & 0.03 & 21.18 & 0.03 & 22.16 & 0.03 & 22.12 & 0.03 & 21.38 & 0.03 & 30.0 & 2.0 & 20316.0 & 3285.4 & 0.05 & 0.03 & -1.65 & 3.0\\
  188.57021\_8.177194 & ngc4535 & 188.57021 & 8.17719 & 4726.79 & 1301.42 & 21.31 & 0.04 & 21.61 & 0.04 & 22.87 & 0.04 & 22.89 & 0.04 & 22.45 & 0.05 & 7.0 & 1.0 & 2234.13 & 103.47 & 0.06 & 0.03 & -1.21 & 3.0\\
  188.574173\_8.209706 & ngc4535 & 188.57417 & 8.20971 & 4370.95 & 4255.14 & 19.03 & 0.05 & 19.62 & 0.05 & 21.08 & 0.05 & 21.17 & 0.05 & 21.0 & 0.04 & 1.0 & 2.0 & 35345.0 & 9319.55 & 0.2 & 0.02 & -1.27 & 3.0\\
  188.573535\_8.211118 & ngc4535 & 188.57354 & 8.21112 & 4428.59 & 4383.53 & 19.76 & 0.03 & 20.03 & 0.03 & 21.36 & 0.02 & 21.34 & 0.03 & 21.09 & 0.04 & 1.0 & 1.0 & 44640.56 & 4052.34 & 0.34 & 0.03 & -1.01 & 3.0\\
  188.56981\_8.17861 & ngc4535 & 188.56981 & 8.17861 & 4763.1 & 1430.25 & 20.28 & 0.02 & 20.61 & 0.02 & 21.94 & 0.03 & 21.98 & 0.03 & 21.15 & 0.03 & 9.0 & 0.0 & 7787.57 & 933.44 & 0.02 & 0.03 & -1.42 & 3.0\\
  188.860137\_14.519198 & ngc4548 & 188.86014 & 14.5192 & 3408.1 & 5252.62 & 24.03 & 0.28 & 23.53 & 0.16 & 23.34 & 0.04 & 22.7 & 0.02 & 21.62 & 0.02 & 210.0 & 818.0 & 115236.13 & 21084.47 & 0.46 & 0.32 & -1.66 & 1.0\\
  188.86335\_14.497687 & ngc4548 & 188.86335 & 14.49769 & 3125.31 & 3297.91 & 23.87 & 0.32 & 23.26 & 0.16 & 22.74 & 0.03 & 22.17 & 0.02 & 21.03 & 0.02 & 349.0 & 26.0 & 211767.82 & 29194.77 & 0.39 & 0.07 & -1.75 & 1.0\\
  188.861536\_14.499697 & ngc4548 & 188.86154 & 14.4997 & 3284.91 & 3480.62 & 23.4 & 0.26 & 22.31 & 0.09 & 21.85 & 0.02 & 21.09 & 0.01 & 19.85 & 0.01 & 890.0 & 1929.0 & 857218.32 & 306035.15 & 0.29 & 0.25 & -1.85 & 1.0\\
  188.835264\_14.509127 & ngc4548 & 188.83526 & 14.50913 & 5595.77 & 4337.62 &  & -0.36 & 23.34 & 0.14 & 22.81 & 0.03 & 22.0 & 0.01 & 20.67 & 0.01 & 828.0 & 3839.0 & 442843.33 & 501323.2 & 0.37 & 0.27 & -1.61 & 1.0\\
  188.862491\_14.494777 & ngc4548 & 188.86249 & 14.49478 & 3200.86 & 3033.46 & 24.0 & 0.35 & 22.77 & 0.1 & 22.6 & 0.03 & 21.81 & 0.02 & 20.54 & 0.02 & 2271.0 & 3954.0 & 537343.24 & 526266.21 & 0.06 & 0.06 & -1.85 & 1.0\\
  188.843485\_14.516919 & ngc4548 & 188.84348 & 14.51692 & 4872.62 & 5045.51 & 22.83 & 0.1 & 22.14 & 0.05 & 22.35 & 0.02 & 21.82 & 0.01 & 20.76 & 0.01 & 118.0 & 9.0 & 196477.12 & 30016.28 & 0.46 & 0.06 & -1.7 & 1.0\\
  188.860983\_14.501728 & ngc4548 & 188.86098 & 14.50173 & 3333.55 & 3665.12 & 23.93 & 0.33 & 22.76 & 0.1 & 22.6 & 0.03 & 22.02 & 0.02 & 20.88 & 0.02 & 1276.0 & 171.0 & 235173.64 & 427.45 & 0.03 & 0.07 & -1.88 & 1.0\\
  188.861058\_14.497215 & ngc4548 & 188.86106 & 14.49722 & 3326.9 & 3254.95 & 24.05 & 0.38 & 22.34 & 0.08 & 22.02 & 0.02 & 21.33 & 0.02 & 20.0 & 0.02 & 2623.0 & 510.0 & 1022787.24 & 273954.41 & 0.07 & 0.03 & -1.71 & 1.0\\
  188.855725\_14.486818 & ngc4548 & 188.85572 & 14.48682 & 3796.09 & 2310.27 & 23.73 & 0.26 & 22.34 & 0.06 & 22.12 & 0.02 & 21.36 & 0.01 & 20.07 & 0.01 & 2440.0 & 1412.0 & 897967.44 & 229026.63 & 0.06 & 0.19 & -1.64 & 1.0\\
  188.8638\_14.482152 & ngc4548 & 188.8638 & 14.48215 & 3085.6 & 1886.26 & 23.61 & 0.22 & 22.54 & 0.07 & 22.34 & 0.02 & 21.55 & 0.01 & 20.24 & 0.01 & 1276.0 & 2765.0 & 523117.81 & 568396.98 & 0.16 & 0.12 & -1.71 & 1.0\\
  188.853191\_14.485031 & ngc4548 & 188.85319 & 14.48503 & 4019.0 & 2147.93 & 23.88 & 0.3 & 22.06 & 0.05 & 21.77 & 0.01 & 20.97 & 0.01 & 19.64 & 0.01 & 6225.0 & 4641.0 & 2323510.04 & 942973.03 & 0.0 & 0.23 & -1.64 & 1.0\\
  188.83743\_14.510993 & ngc4548 & 188.83743 & 14.51099 & 5405.25 & 4507.09 & 26.63 & 3.23 & 26.81 & 3.11 & 25.12 & 0.18 & 23.91 & 0.05 & 22.71 & 0.04 & 10308.0 & 9771.0 & 201754.71 & 122789.02 & 0.0 & 0.55 & -1.38 & 2.0\\
  188.866007\_14.509207 & ngc4548 & 188.86601 & 14.50921 & 2891.57 & 4344.52 & 20.17 & 0.02 & 20.56 & 0.02 & 22.03 & 0.02 & 22.04 & 0.02 & 21.8 & 0.03 & 1.0 & 2.0 & 19778.46 & 5673.15 & 0.26 & 0.01 & -0.95 & 2.0\\
  188.872082\_14.505824 & ngc4548 & 188.87208 & 14.50582 & 2357.36 & 4037.3 & 20.95 & 0.03 & 21.07 & 0.02 & 22.42 & 0.02 & 22.32 & 0.02 & 21.91 & 0.04 & 1.0 & 2.0 & 24168.7 & 6949.16 & 0.41 & 0.01 & -0.9 & 2.0\\
  188.865027\_14.509326 & ngc4548 & 188.86503 & 14.50933 & 2977.93 & 4355.43 & 19.77 & 0.01 & 20.17 & 0.01 & 21.6 & 0.01 & 21.71 & 0.01 & 21.67 & 0.03 & 1.0 & 3.0 & 22344.67 & 16243.56 & 0.21 & 0.12 & -1.92 & 2.0\\
  188.840375\_14.494038 & ngc4548 & 188.84038 & 14.49404 & 5146.63 & 2966.97 & 18.63 & 0.01 & 19.06 & 0.01 & 20.57 & 0.02 & 20.58 & 0.01 & 20.39 & 0.02 & 1.0 & 2.0 & 71486.63 & 22473.93 & 0.24 & 0.0 & -0.96 & 2.0\\
  188.871779\_14.502622 & ngc4548 & 188.87178 & 14.50262 & 2383.79 & 3746.42 & 22.27 & 0.08 & 21.9 & 0.04 & 21.97 & 0.02 & 21.42 & 0.01 & 20.33 & 0.01 & 110.0 & 26.0 & 288401.21 & 26773.91 & 0.48 & 0.01 & -1.76 & 2.0\\
  188.877209\_14.500522 & ngc4548 & 188.87721 & 14.50052 & 1906.01 & 3555.39 & 18.76 & 0.01 & 19.04 & 0.01 & 20.41 & 0.01 & 20.38 & 0.01 & 20.19 & 0.01 & 1.0 & 0.0 & 106343.53 & 12749.23 & 0.32 & 0.03 & -1.69 & 2.0\\
  188.85476\_14.476916 & ngc4548 & 188.85476 & 14.47692 & 3880.48 & 1410.63 & 20.26 & 0.02 & 20.72 & 0.02 & 22.32 & 0.02 & 22.44 & 0.02 & 22.47 & 0.04 & 1.0 & 0.0 & 9271.78 & 1408.63 & 0.14 & 0.04 & -1.61 & 2.0\\
  188.840555\_14.493293 & ngc4548 & 188.84056 & 14.49329 & 5130.7 & 2898.63 & 20.24 & 0.02 & 20.56 & 0.02 & 21.97 & 0.02 & 21.95 & 0.02 & 21.83 & 0.04 & 1.0 & 2.0 & 21709.7 & 9514.3 & 0.28 & 0.05 & -1.94 & 2.0\\
  188.8552\_14.476984 & ngc4548 & 188.8552 & 14.47698 & 3842.34 & 1416.95 & 21.06 & 0.03 & 21.5 & 0.03 & 23.05 & 0.04 & 23.15 & 0.03 & 22.6 & 0.05 & 1.0 & 2.0 & 7342.09 & 3226.06 & 0.24 & 0.05 & -1.6 & 3.0\\
  188.848058\_14.478908 & ngc4548 & 188.84806 & 14.47891 & 4470.17 & 1591.05 & 22.5 & 0.09 & 23.22 & 0.14 & 24.23 & 0.08 & 24.14 & 0.07 & 23.42 & 0.08 & 11.0 & 19.0 & 1194.09 & 1699.39 & 0.01 & 0.01 & -1.11 & 3.0\\
  188.839937\_14.515526 & ngc4548 & 188.83994 & 14.51553 & 5184.96 & 4919.85 & 21.17 & 0.03 & 21.71 & 0.04 & 23.24 & 0.04 & 23.38 & 0.04 & 23.63 & 0.11 & 3.0 & 2.0 & 2051.39 & 654.28 & 0.08 & 0.02 & -1.18 & 3.0\\
  188.840269\_14.51581 & ngc4548 & 188.84027 & 14.51581 & 5155.48 & 4944.64 & 21.84 & 0.06 & 21.85 & 0.04 & 22.91 & 0.03 & 22.89 & 0.03 & 22.26 & 0.04 & 1.0 & 6.0 & 21671.62 & 18318.14 & 0.53 & 0.35 & -1.12 & 3.0\\
  188.884931\_14.486254 & ngc4548 & 188.88493 & 14.48625 & 1226.97 & 2259.24 & 21.06 & 0.04 & 21.42 & 0.04 & 22.93 & 0.04 & 22.96 & 0.04 & 22.75 & 0.07 & 1.0 & 1.0 & 7935.17 & 391.46 & 0.24 & 0.04 & -0.95 & 3.0\\
  188.842619\_14.491571 & ngc4548 & 188.84262 & 14.49157 & 4949.27 & 2742.26 & 19.64 & 0.02 & 20.06 & 0.02 & 21.47 & 0.02 & 21.51 & 0.01 & 21.11 & 0.02 & 7.0 & 6.0 & 7215.07 & 29846.06 & 0.0 & 0.29 & -1.09 & 3.0\\
  188.870029\_14.507277 & ngc4548 & 188.87003 & 14.50728 & 2537.69 & 4169.13 & 20.7 & 0.03 & 21.17 & 0.03 & 22.17 & 0.02 & 22.16 & 0.02 & 21.58 & 0.03 & 8.0 & 26.0 & 6027.87 & 14058.69 & 0.09 & 0.08 & -0.76 & 3.0\\
  188.842056\_14.491385 & ngc4548 & 188.84206 & 14.49138 & 4998.36 & 2725.65 & 20.48 & 0.02 & 20.75 & 0.02 & 22.11 & 0.02 & 22.07 & 0.02 & 21.81 & 0.04 & 1.0 & 0.0 & 24203.89 & 3609.32 & 0.34 & 0.04 & -0.84 & 3.0\\
  188.877453\_14.500286 & ngc4548 & 188.87745 & 14.50029 & 1884.48 & 3534.61 & 20.86 & 0.04 & 21.35 & 0.05 & 22.83 & 0.05 & 23.04 & 0.07 & 22.92 & 0.1 & 1.0 & 3.0 & 5967.35 & 4542.73 & 0.16 & 0.15 & -1.27 & 3.0\\
  188.842129\_14.490007 & ngc4548 & 188.84213 & 14.49001 & 4991.65 & 2600.34 & 20.95 & 0.1 & 21.62 & 0.1 & 22.39 & 0.07 & 21.96 & 0.04 & 21.06 & 0.03 & 12.0 & 9.0 & 16797.21 & 11185.7 & 0.23 & 0.03 & -1.52 & 3.0\\
  189.220977\_13.184923 & ngc4569 & 189.22098 & 13.18492 & 2295.38 & 5415.47 & 22.56 & 0.1 & 22.06 & 0.06 & 21.96 & 0.02 & 21.79 & 0.01 & 21.17 & 0.02 & 403.0 & 28.0 & 101287.34 & 10320.21 & 0.0 & 0.05 & -1.71 & 1.0\\
  189.213344\_13.174785 & ngc4569 & 189.21334 & 13.17478 & 2970.56 & 4494.52 & 23.05 & 0.17 & 22.23 & 0.07 & 21.87 & 0.02 & 21.47 & 0.01 & 20.53 & 0.01 & 621.0 & 269.0 & 267062.39 & 42860.57 & 0.12 & 0.05 & -1.78 & 1.0\\
  189.207334\_13.165 & ngc4569 & 189.20733 & 13.165 & 3502.24 & 3605.12 & 24.56 & 0.57 & 23.35 & 0.17 & 22.87 & 0.05 & 21.93 & 0.03 & 20.48 & 0.02 & 1187.0 & 838.0 & 471133.09 & 123951.35 & 0.32 & 0.38 & -1.68 & 1.0\\
  189.210454\_13.176995 & ngc4569 & 189.21045 & 13.177 & 3225.97 & 4694.99 & 23.44 & 0.24 & 23.02 & 0.13 & 22.66 & 0.03 & 22.31 & 0.02 & 21.54 & 0.03 & 465.0 & 35.0 & 90985.12 & 16160.44 & 0.1 & 0.08 & -1.78 & 1.0\\
  189.196283\_13.151256 & ngc4569 & 189.19628 & 13.15126 & 4479.92 & 2356.7 & 22.83 & 0.14 & 22.64 & 0.09 & 22.45 & 0.03 & 22.25 & 0.02 & 21.61 & 0.03 & 375.0 & 73.0 & 64167.11 & 11323.55 & 0.01 & 0.0 & -1.75 & 1.0\\
  189.195895\_13.147169 & ngc4569 & 189.1959 & 13.14717 & 4514.23 & 1985.15 & 23.34 & 0.21 & 22.53 & 0.08 & 22.44 & 0.02 & 21.68 & 0.01 & 20.45 & 0.01 & 147.0 & 1327.0 & 327913.14 & 69962.06 & 0.59 & 0.52 & -1.45 & 1.0\\
  189.198073\_13.144201 & ngc4569 & 189.19807 & 13.1442 & 4321.54 & 1715.38 & 21.6 & 0.05 & 21.25 & 0.03 & 21.14 & 0.01 & 20.91 & 0.01 & 20.35 & 0.01 & 403.0 & 30.0 & 221392.83 & 22252.3 & 0.0 & 0.01 & -1.74 & 1.0\\
  189.200241\_13.167733 & ngc4569 & 189.20024 & 13.16773 & 4129.55 & 3853.53 & 24.29 & 0.5 & 23.9 & 0.29 & 23.23 & 0.05 & 22.76 & 0.03 & 21.96 & 0.04 & 500.0 & 125.0 & 70778.04 & 13506.72 & 0.15 & 0.0 & -1.76 & 1.0\\
  189.224068\_13.18112 & ngc4569 & 189.22407 & 13.18112 & 2021.89 & 5069.93 & 22.06 & 0.07 & 20.76 & 0.02 & 20.54 & 0.01 & 19.77 & 0.0 & 18.49 & 0.0 & 2113.0 & 0.0 & 3207256.53 & 461675.52 & 0.07 & 0.04 & -1.63 & 1.0\\
  189.224768\_13.180594 & ngc4569 & 189.22477 & 13.18059 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & -1.55 & 1.0\\
  189.213649\_13.178158 & ngc4569 & 189.21365 & 13.17816 & 2943.46 & 4800.62 & 23.63 & 0.27 & 23.36 & 0.17 & 23.1 & 0.05 & 22.63 & 0.03 & 21.75 & 0.04 & 302.0 & 131.0 & 71523.16 & 3015.8 & 0.23 & 0.11 & -1.61 & 2.0\\
  189.211892\_13.179985 & ngc4569 & 189.21189 & 13.17998 & 3098.73 & 4966.74 & 19.37 & 0.02 & 19.42 & 0.02 & 20.49 & 0.02 & 20.31 & 0.02 & 19.88 & 0.02 & 3.0 & 1.0 & 126901.28 & 76260.71 & 0.51 & 0.12 & -1.53 & 2.0\\
  189.20598\_13.173487 & ngc4569 & 189.20598 & 13.17349 & 3621.98 & 4376.5 & 22.73 & 0.14 & 22.05 & 0.06 & 21.72 & 0.02 & 21.43 & 0.01 & 20.68 & 0.02 & 577.0 & 202.0 & 195300.5 & 5603.92 & 0.03 & 0.1 & -1.68 & 2.0\\
  189.204331\_13.167196 & ngc4569 & 189.20433 & 13.1672 & 3768.2 & 3804.48 & 19.45 & 0.01 & 19.76 & 0.01 & 21.03 & 0.01 & 21.01 & 0.01 & 20.67 & 0.02 & 7.0 & 1.0 & 11817.79 & 942.44 & 0.05 & 0.02 & -1.69 & 2.0\\
  189.205253\_13.173334 & ngc4569 & 189.20525 & 13.17333 & 3686.33 & 4362.35 & 22.96 & 0.15 & 23.08 & 0.14 & 22.94 & 0.04 & 22.8 & 0.03 & 22.41 & 0.06 & 243.0 & 18.0 & 26316.85 & 3776.71 & 0.0 & 0.03 & -1.6 & 2.0\\
  189.202334\_13.15809 & ngc4569 & 189.20233 & 13.15809 & 3943.96 & 2976.71 & 23.05 & 0.18 & 22.33 & 0.08 & 22.41 & 0.03 & 22.13 & 0.02 & 21.33 & 0.03 & 281.0 & 0.0 & 86986.34 & 14312.81 & 0.14 & 0.05 & -1.67 & 2.0\\
  189.202061\_13.159561 & ngc4569 & 189.20206 & 13.15956 & 3968.77 & 3111.02 & 20.94 & 0.03 & 20.66 & 0.02 & 21.26 & 0.01 & 20.92 & 0.01 & 19.93 & 0.01 & 6.0 & 4.0 & 56011.98 & 195814.62 & 0.58 & 0.27 & -1.76 & 2.0\\
  189.200282\_13.165157 & ngc4569 & 189.20028 & 13.16516 & 4126.29 & 3619.51 & 23.33 & 0.21 & 22.77 & 0.11 & 22.27 & 0.02 & 22.07 & 0.02 & 21.42 & 0.03 & 500.0 & 121.0 & 96203.33 & 13624.3 & 0.03 & 0.01 & -1.72 & 2.0\\
  189.191689\_13.15365 & ngc4569 & 189.19169 & 13.15365 & 4886.72 & 2573.64 & 23.09 & 0.19 & 22.9 & 0.12 & 22.64 & 0.03 & 22.46 & 0.02 & 21.8 & 0.03 & 403.0 & 97.0 & 56536.17 & 9452.18 & 0.01 & 0.0 & -1.62 & 2.0\\
  189.191991\_13.153854 & ngc4569 & 189.19199 & 13.15385 & 4859.52 & 2592.42 & 23.08 & 0.17 & 23.49 & 0.19 & 23.2 & 0.04 & 22.96 & 0.03 & 22.29 & 0.05 & 261.0 & 114.0 & 31555.78 & 1271.64 & 0.08 & 0.1 & -1.68 & 2.0\\
  189.212201\_13.179812 & ngc4569 & 189.2122 & 13.17981 & 3071.6294547358293 & 4951.078773847782 & 22.29 & 0.1 & 22.37 & 0.1 & 23.2 & 0.08 & 22.76 & 0.06 & 21.83 & 0.05 & 8.0 & 32.0 & 7980.66 & 11526.78 & 0.4 & 0.19 & -0.92 & 3.0\\
  189.201826\_13.153873 & ngc4569 & 189.20183 & 13.15387 & 3989.53 & 2593.89 & 22.99 & 0.62 & 23.1 & 0.59 & 23.3 & 0.28 & 23.08 & 0.23 & 23.19 & 0.72 & 182.0 & 283.0 & 16736.43 & 21702.64 & 0.0 & 0.07 & -0.91 & 3.0\\
  189.202005\_13.153999 & ngc4569 & 189.202 & 13.154 & 3973.62 & 2605.04 & 20.17 & 0.04 & 20.53 & 0.04 & 22.01 & 0.04 & 22.17 & 0.06 & 22.68 & 0.17 & 4.0 & 1.0 & 2817.33 & 5012.36 & 0.02 & 0.14 & -0.62 & 3.0\\
  189.212682\_13.179589 & ngc4569 & 189.21268 & 13.17959 & 3029.16 & 4931.09 & 21.46 & 0.04 & 21.46 & 0.03 & 22.44 & 0.03 & 22.21 & 0.02 & 21.72 & 0.04 & 3.0 & 2.0 & 26217.55 & 17043.26 & 0.57 & 0.18 & -0.83 & 3.0\\
  189.213552\_13.179413 & ngc4569 & 189.21355 & 13.17941 & 2951.48 & 4914.56 & 22.2 & 0.08 & 22.19 & 0.06 & 23.13 & 0.05 & 22.92 & 0.04 & 22.33 & 0.07 & 3.0 & 50.0 & 15437.81 & 464.84 & 0.6 & 0.5 & -1.3 & 3.0\\
  189.202505\_13.159603 & ngc4569 & 189.2025 & 13.1596 & 3929.32 & 3114.61 & 22.95 & 0.24 & 22.81 & 0.16 & 22.75 & 0.06 & 22.59 & 0.05 & 21.97 & 0.09 & 302.0 & 133.0 & 38596.58 & 10550.55 & 0.0 & 0.19 & -0.68 & 3.0\\
  189.211723\_13.174107 & ngc4569 & 189.21172 & 13.17411 & 3114.57 & 4433.42 & 22.33 & 0.14 & 22.12 & 0.14 & 23.36 & 0.26 & 23.15 & 0.37 & 21.99 & 0.33 & 1.0 & 70.0 & 26366.48 & 8292.2 & 0.65 & 0.55 & -0.83 & 3.0\\
  189.201745\_13.154549 & ngc4569 & 189.20174 & 13.15455 & 3996.65 & 2655.27 & 21.74 & 0.07 & 21.62 & 0.05 & 22.45 & 0.04 & 22.36 & 0.04 & 21.88 & 0.05 & 5.0 & 2.0 & 8347.15 & 16232.37 & 0.4 & 0.19 & -1.24 & 3.0\\
  189.212395\_13.177303 & ngc4569 & 189.2124 & 13.1773 & 3054.28 & 4723.01 & 21.85 & 0.06 & 21.93 & 0.05 & 22.7 & 0.05 & 22.54 & 0.06 & 21.89 & 0.09 & 6.0 & 89.0 & 6156.66 & 15482.06 & 0.35 & 0.35 & -0.93 & 3.0\\
  189.214118\_13.177682 & ngc4569 & 189.21412 & 13.17768 & 2902.6 & 4757.73 & 20.97 & 0.04 & 21.29 & 0.04 & 22.69 & 0.05 & 22.76 & 0.05 & 22.29 & 0.06 & 8.0 & 1.0 & 2672.14 & 225.53 & 0.0 & 0.03 & -1.23 & 3.0\\
  189.224846\_14.209821 & ngc4571 & 189.22485 & 14.20982 & 4279.58 & 2497.28 & 23.01 & 0.15 & 21.94 & 0.05 & 22.05 & 0.02 & 21.43 & 0.01 & 20.3 & 0.01 & 1276.0 & 426.0 & 317646.5 & 115135.67 & 0.0 & 0.0 & -1.78 & 1.0\\
  189.233382\_14.215918 & ngc4571 & 189.23338 & 14.21592 & 3527.93 & 3051.14 & 23.51 & 0.22 & 22.99 & 0.12 & 23.01 & 0.03 & 22.44 & 0.02 & 21.24 & 0.02 & 110.0 & 86.0 & 115809.86 & 8406.79 & 0.54 & 0.09 & -1.84 & 1.0\\
  189.241192\_14.218449 & ngc4571 & 189.24119 & 14.21845 & 2839.89 & 3281.26 & 23.0 & 0.15 & 22.46 & 0.07 & 22.23 & 0.02 & 21.68 & 0.01 & 20.62 & 0.01 & 243.0 & 81.0 & 219922.98 & 16686.39 & 0.39 & 0.04 & -1.79 & 1.0\\
  189.233973\_14.22857 & ngc4571 & 189.23397 & 14.22857 & 3475.62 & 4201.33 & 23.51 & 0.2 & 22.83 & 0.09 & 22.66 & 0.03 & 21.94 & 0.01 & 20.67 & 0.01 & 158.0 & 38.0 & 245398.67 & 8000.36 & 0.59 & 0.06 & -1.72 & 1.0\\
  189.235398\_14.219561 & ngc4571 & 189.2354 & 14.21956 & 3350.12 & 3382.26 & 21.05 & 0.03 & 21.18 & 0.03 & 22.6 & 0.03 & 22.62 & 0.03 & 22.41 & 0.05 & 1.0 & 2.0 & 11597.0 & 5082.56 & 0.32 & 0.05 & -1.86 & 1.0\\
  189.234627\_14.230723 & ngc4571 & 189.23463 & 14.23072 & 3417.86 & 4396.41 &  & -1.13 & 24.15 & 0.3 & 24.11 & 0.07 & 23.17 & 0.03 & 21.96 & 0.03 & 5390.0 & 4673.0 & 216023.62 & 114575.06 & 0.0 & 0.35 & -1.67 & 1.0\\
  189.213528\_14.232532 & ngc4571 & 189.21353 & 14.23253 & 5276.32 & 4561.08 & 25.45 & 1.13 & 23.45 & 0.15 & 23.48 & 0.04 & 22.58 & 0.02 & 21.33 & 0.02 & 2623.0 & 5681.0 & 254564.13 & 284138.1 & 0.07 & 0.06 & -1.44 & 1.0\\
  189.245108\_14.225455 & ngc4571 & 189.24511 & 14.22545 & 2494.87 & 3918.06 & 20.52 & 0.02 & 20.8 & 0.02 & 21.69 & 0.01 & 21.68 & 0.01 & 21.0 & 0.01 & 34.0 & 3.0 & 30372.63 & 4168.63 & 0.06 & 0.05 & -1.55 & 1.0\\
  189.249977\_14.235152 & ngc4571 & 189.24998 & 14.23515 & 2066.14 & 4799.22 & 24.58 & 0.55 & 23.33 & 0.13 & 23.45 & 0.05 & 22.64 & 0.02 & 21.4 & 0.02 & 5.0 & 1271.0 & 35601.53 & 90638.11 & 1.04 & 0.96 & -1.5 & 1.0\\
  189.226369\_14.221155 & ngc4571 & 189.22637 & 14.22116 & 4145.35 & 3527.31 & 23.3 & 0.17 & 22.63 & 0.08 & 22.49 & 0.02 & 21.78 & 0.01 & 20.71 & 0.01 & 196.0 & 909.0 & 239688.57 & 10616.26 & 0.5 & 0.41 & -1.8 & 1.0\\
  189.245427\_14.206889 & ngc4571 & 189.24543 & 14.20689 & 2467.05 & 2230.73 & 21.91 & 0.05 & 22.25 & 0.06 & 23.47 & 0.05 & 23.26 & 0.03 & 22.7 & 0.04 & 8.0 & 6.0 & 1879.06 & 1418.18 & 0.11 & 0.04 & -1.7 & 2.0\\
  189.23578\_14.221247 & ngc4571 & 189.23578 & 14.22125 & 3316.65 & 3535.53 & 20.86 & 0.03 & 21.01 & 0.03 & 22.05 & 0.02 & 22.02 & 0.02 & 21.59 & 0.03 & 4.0 & 2.0 & 9084.45 & 20950.6 & 0.36 & 0.15 & -1.89 & 2.0\\
  189.231254\_14.230328 & ngc4571 & 189.23125 & 14.23033 & 3715.16 & 4360.74 & 20.13 & 0.02 & 20.52 & 0.02 & 21.79 & 0.02 & 21.8 & 0.02 & 21.76 & 0.03 & 4.0 & 1.0 & 5791.8 & 9263.46 & 0.17 & 0.13 & -1.55 & 2.0\\
  189.233944\_14.218847 & ngc4571 & 189.23394 & 14.21885 & 3478.14 & 3317.46 & 21.39 & 0.04 & 21.33 & 0.03 & 22.45 & 0.02 & 22.5 & 0.02 & 22.28 & 0.05 & 4.0 & 0.0 & 4965.36 & 812.19 & 0.32 & 0.04 & -1.83 & 2.0\\
  189.252307\_14.211536 & ngc4571 & 189.25231 & 14.21154 & 1860.06 & 2653.62 & 20.67 & 0.02 & 20.73 & 0.02 & 21.97 & 0.02 & 22.0 & 0.01 & 21.59 & 0.02 & 1.0 & 2.0 & 29038.87 & 12631.02 & 0.42 & 0.05 & -1.37 & 2.0\\
  189.238071\_14.200557 & ngc4571 & 189.23807 & 14.20056 & 3114.66 & 1655.52 & 19.78 & 0.01 & 20.16 & 0.01 & 21.72 & 0.01 & 21.84 & 0.01 & 21.85 & 0.02 & 1.0 & 0.0 & 14885.03 & 1818.29 & 0.17 & 0.03 & -1.55 & 2.0\\
  189.243847\_14.210223 & ngc4571 & 189.24385 & 14.21022 & 2605.51 & 2533.6 & 20.57 & 0.02 & 21.07 & 0.03 & 22.54 & 0.02 & 22.66 & 0.02 & 22.73 & 0.05 & 1.0 & 1.0 & 6617.57 & 2065.75 & 0.16 & 0.04 & -1.43 & 2.0\\
  189.217913\_14.212464 & ngc4571 & 189.21791 & 14.21246 & 4890.07 & 2737.39 & 19.19 & 0.01 & 19.62 & 0.01 & 21.06 & 0.02 & 21.13 & 0.02 & 21.01 & 0.03 & 1.0 & 1.0 & 34825.19 & 10802.75 & 0.23 & 0.04 & -0.9 & 2.0\\
  189.233904\_14.218183 & ngc4571 & 189.2339 & 14.21818 & 3481.67 & 3257.08 & 20.46 & 0.02 & 20.94 & 0.02 & 22.49 & 0.03 & 22.57 & 0.03 & 22.74 & 0.09 & 1.0 & 0.0 & 6566.04 & 1190.58 & 0.14 & 0.04 & -1.68 & 2.0\\
  189.255575\_14.213901 & ngc4571 & 189.25558 & 14.2139 & 1572.75 & 2868.23 & 21.31 & 0.04 & 21.74 & 0.04 & 23.34 & 0.04 & 23.55 & 0.04 & 23.36 & 0.07 & 1.0 & 1.0 & 2992.99 & 139.78 & 0.14 & 0.04 & -1.7 & 2.0\\
  189.233558\_14.232858 & ngc4571 & 189.23356 & 14.23286 & 3512.21 & 4590.7 & 22.1 & 0.07 & 22.49 & 0.08 & 23.5 & 0.05 & 23.14 & 0.04 & 22.47 & 0.05 & 15.0 & 19.0 & 4406.85 & 3046.88 & 0.13 & 0.05 & -1.11 & 3.0\\
  189.232905\_14.231459 & ngc4571 & 189.2329 & 14.23146 & 3569.74 & 4463.71 & 20.76 & 0.06 & 21.03 & 0.06 & 21.87 & 0.04 & 21.86 & 0.03 & 21.32 & 0.03 & 53.0 & 21.0 & 27102.64 & 5921.85 & 0.0 & 0.03 & -1.68 & 3.0\\
  189.223536\_14.220784 & ngc4571 & 189.22354 & 14.22078 & 4395.15 & 3494.02 & 20.05 & 0.02 & 20.26 & 0.02 & 21.46 & 0.02 & 21.37 & 0.02 & 20.97 & 0.03 & 1.0 & 0.0 & 51249.17 & 8373.77 & 0.43 & 0.04 & -1.0 & 3.0\\
  189.214847\_14.213285 & ngc4571 & 189.21485 & 14.21328 & 5160.01 & 2812.46 & 22.68 & 0.12 & 23.2 & 0.14 & 24.26 & 0.11 & 24.17 & 0.09 & 23.68 & 0.1 & 8.0 & 10.0 & 723.57 & 915.53 & 0.07 & 0.04 & -0.61 & 3.0\\
  189.218021\_14.212491 & ngc4571 & 189.21802 & 14.21249 & 4880.66 & 2740.55 & 20.04 & 0.03 & 20.45 & 0.03 & 21.97 & 0.03 & 22.16 & 0.03 & 22.37 & 0.07 & 3.0 & 1.0 & 5807.75 & 2879.59 & 0.1 & 0.06 & -1.02 & 3.0\\
  189.224744\_14.211093 & ngc4571 & 189.22474 & 14.21109 & 4288.44 & 2612.91 & 22.31 & 0.09 & 22.99 & 0.13 & 24.12 & 0.09 & 24.18 & 0.08 & 23.81 & 0.13 & 7.0 & 0.0 & 496.53 & 126.6 & 0.0 & 0.06 & -1.63 & 3.0\\
  189.227653\_14.227186 & ngc4571 & 189.22765 & 14.22719 & 4032.34 & 4075.42 & 21.37 & 0.06 & 21.52 & 0.05 & 22.64 & 0.04 & 22.56 & 0.04 & 21.95 & 0.04 & 7.0 & 21.0 & 4029.94 & 5186.44 & 0.19 & 0.19 & -1.12 & 3.0\\
  189.230898\_14.208871 & ngc4571 & 189.2309 & 14.20887 & 3746.12 & 2410.47 & 19.34 & 0.01 & 19.76 & 0.01 & 21.28 & 0.02 & 21.4 & 0.01 & 21.28 & 0.02 & 1.0 & 0.0 & 24507.14 & 4073.43 & 0.19 & 0.04 & -0.76 & 3.0\\
  189.22689\_14.22712 & ngc4571 & 189.22689 & 14.22712 & 4099.37 & 4069.08 & 20.3 & 0.02 & 20.67 & 0.02 & 21.97 & 0.02 & 22.11 & 0.02 & 21.94 & 0.03 & 1.0 & 1.0 & 16216.33 & 1471.36 & 0.27 & 0.03 & -0.82 & 3.0\\
  189.240396\_14.236765 & ngc4571 & 189.2404 & 14.23676 & 2909.88 & 4945.52 & 21.91 & 0.05 & 22.25 & 0.06 & 23.84 & 0.07 & 23.94 & 0.07 & 24.06 & 0.16 & 1.0 & 0.0 & 2025.78 & 585.75 & 0.16 & 0.06 & -0.71 & 3.0\\
  190.975186\_13.12208 & ngc4654 & 190.97519 & 13.12208 & 4140.26 & 2653.26 & 22.93 & 0.14 & 22.18 & 0.06 & 22.13 & 0.02 & 21.52 & 0.01 & 20.41 & 0.01 & 182.0 & 64.0 & 631198.03 & 72658.94 & 0.48 & 0.05 & -1.54 & 1.0\\
  190.981905\_13.146503 & ngc4654 & 190.9819 & 13.1465 & 3545.77 & 4872.51 & 23.59 & 0.23 & 23.29 & 0.14 & 22.98 & 0.04 & 22.54 & 0.02 & 21.53 & 0.02 & 261.0 & 103.0 & 186374.87 & 20127.16 & 0.32 & 0.06 & -1.6 & 1.0\\
  190.984691\_13.126297 & ngc4654 & 190.98469 & 13.1263 & 3299.12 & 3036.59 & 22.74 & 0.14 & 21.99 & 0.07 & 21.92 & 0.03 & 21.57 & 0.02 & 20.59 & 0.03 & 281.0 & 20.0 & 398655.61 & 73515.81 & 0.25 & 0.07 & -1.69 & 1.0\\
  190.977564\_13.123286 & ngc4654 & 190.97756 & 13.12329 & 3929.76 & 2762.77 & 25.02 & 0.99 & 22.95 & 0.12 & 23.13 & 0.04 & 22.59 & 0.03 & 21.49 & 0.02 & 1276.0 & 1149.0 & 236436.03 & 33280.08 & 0.0 & 0.5 & -1.83 & 1.0\\
  190.963481\_13.133425 & ngc4654 & 190.96348 & 13.13342 & 5175.92 & 3684.25 & 21.81 & 0.06 & 21.56 & 0.04 & 21.29 & 0.01 & 21.04 & 0.01 & 20.26 & 0.01 & 324.0 & 81.0 & 456449.44 & 66928.38 & 0.11 & 0.11 & -1.72 & 1.0\\
  190.973755\_13.136363 & ngc4654 & 190.97376 & 13.13636 & 4266.85 & 3951.23 & 21.31 & 0.04 & 21.31 & 0.03 & 21.83 & 0.02 & 21.64 & 0.01 & 20.97 & 0.02 & 88.0 & 83.0 & 135222.97 & 92437.63 & 0.13 & 0.38 & -1.77 & 1.0\\
  190.975812\_13.123355 & ngc4654 & 190.97581 & 13.12335 & 4084.13 & 2769.4 & 23.51 & 0.24 & 22.91 & 0.11 & 22.38 & 0.02 & 22.08 & 0.02 & 21.38 & 0.02 & 500.0 & 217.0 & 210654.67 & 29475.86 & 0.08 & 0.05 & -1.69 & 1.0\\
  190.972628\_13.110767 & ngc4654 & 190.97263 & 13.11077 & 4366.66 & 1625.49 & 23.04 & 0.17 & 22.66 & 0.08 & 22.62 & 0.03 & 22.44 & 0.02 & 21.84 & 0.03 & 349.0 & 68.0 & 95749.24 & 15927.45 & 0.0 & 0.0 & -1.78 & 1.0\\
  191.001136\_13.116161 & ngc4654 & 191.00114 & 13.11616 & 1843.98 & 2115.58 & 22.44 & 0.1 & 22.53 & 0.08 & 22.66 & 0.03 & 22.49 & 0.02 & 21.86 & 0.03 & 169.0 & 22.0 & 78255.3 & 12449.32 & 0.09 & 0.02 & -1.74 & 1.0\\
  190.974284\_13.109608 & ngc4654 & 190.97428 & 13.10961 & 4220.1 & 1520.12 & 22.69 & 0.11 & 22.43 & 0.07 & 22.3 & 0.02 & 22.02 & 0.02 & 21.35 & 0.02 & 349.0 & 123.0 & 160780.6 & 21815.39 & 0.05 & 0.14 & -1.6 & 1.0\\
  190.982199\_13.118128 & ngc4654 & 190.9822 & 13.11813 & 3519.69 & 2294.06 & 22.22 & 0.08 & 22.02 & 0.06 & 23.23 & 0.05 & 22.68 & 0.03 & 22.09 & 0.05 & 1.0 & 1.0 & 64622.88 & 4662.55 & 0.68 & 0.04 & -1.48 & 2.0\\
  190.985559\_13.114 & ngc4654 & 190.98556 & 13.114 & 3222.34 & 1919.09 & 21.85 & 0.06 & 22.14 & 0.06 & 22.38 & 0.02 & 22.29 & 0.02 & 21.67 & 0.02 & 136.0 & 9.0 & 75251.8 & 13424.72 & 0.05 & 0.06 & -1.69 & 2.0\\
  190.975085\_13.110737 & ngc4654 & 190.97508 & 13.11074 & 4149.05 & 1622.7 & 19.79 & 0.02 & 20.16 & 0.02 & 21.64 & 0.02 & 21.6 & 0.02 & 21.42 & 0.03 & 1.0 & 1.0 & 54583.3 & 16872.91 & 0.27 & 0.04 & -1.79 & 2.0\\
  190.958898\_13.138888 & ngc4654 & 190.9589 & 13.13889 & 5581.4 & 4180.6 & 24.32 & 0.51 & 23.43 & 0.18 & 23.32 & 0.05 & 23.14 & 0.04 & 22.63 & 0.05 & 403.0 & 122.0 & 54465.22 & 5733.7 & 0.0 & 0.06 & -1.67 & 2.0\\
  190.961423\_13.131578 & ngc4654 & 190.96142 & 13.13158 & 5358.11 & 3516.55 & 23.82 & 0.3 & 24.12 & 0.33 & 23.38 & 0.05 & 22.96 & 0.03 & 22.29 & 0.04 & 465.0 & 184.0 & 89256.38 & 21094.57 & 0.09 & 0.04 & -1.62 & 2.0\\
  191.008673\_13.118587 & ngc4654 & 191.00867 & 13.11859 & 1176.41 & 2336.11 & 24.55 & 0.59 & 23.77 & 0.23 & 23.86 & 0.08 & 23.36 & 0.04 & 22.37 & 0.04 & 169.0 & 452.0 & 82032.01 & 33953.98 & 0.38 & 0.17 & -1.53 & 2.0\\
  190.964925\_13.121915 & ngc4654 & 190.96492 & 13.12192 & 5048.22 & 2638.31 & 25.51 & 1.46 & 23.41 & 0.17 & 23.2 & 0.04 & 22.48 & 0.02 & 21.24 & 0.02 & 2440.0 & 3353.0 & 550532.18 & 461558.24 & 0.04 & 0.03 & -1.69 & 2.0\\
  190.989285\_13.145029 & ngc4654 & 190.98928 & 13.14503 & 2892.49 & 4738.59 & 23.64 & 0.25 & 23.27 & 0.14 & 22.98 & 0.04 & 22.7 & 0.02 & 21.85 & 0.03 & 349.0 & 272.0 & 116655.59 & 29196.95 & 0.14 & 0.07 & -1.57 & 2.0\\
  191.004323\_13.129909 & ngc4654 & 191.00432 & 13.12991 & 1562.12 & 3364.75 & 22.23 & 0.09 & 22.19 & 0.06 & 22.7 & 0.03 & 22.44 & 0.02 & 21.77 & 0.03 & 95.0 & 90.0 & 70315.63 & 49769.52 & 0.15 & 0.37 & -1.7 & 2.0\\
  190.989711\_13.118168 & ngc4654 & 190.98971 & 13.11817 & 2854.62 & 2297.46 & 17.16 & 0.0 & 17.62 & 0.0 & 19.21 & 0.0 & 19.26 & 0.0 & 19.2 & 0.01 & 1.0 & 2.0 & 361402.98 & 113699.67 & 0.18 & 0.0 & -1.4 & 2.0\\
  190.971522\_13.14178 & ngc4654 & 190.97152 & 13.14178 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & -0.86 & 3.0\\
  190.968283\_13.141882 & ngc4654 & 190.96828 & 13.14188 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & -1.67 & 3.0\\
  190.970078\_13.143161 & ngc4654 & 190.97008 & 13.14316 & 4592.19 & 4568.89 & 19.68 & 0.03 & 20.12 & 0.03 & 21.53 & 0.03 & 21.56 & 0.02 & 21.3 & 0.03 & 1.0 & 2.0 & 58895.49 & 16968.71 & 0.27 & 0.01 & -1.39 & 3.0\\
  190.97963\_13.144851 & ngc4654 & 190.97963 & 13.14485 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & -1.83 & 3.0\\
  190.997871\_13.137176 & ngc4654 & 190.99787 & 13.13718 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & -0.59 & 3.0\\
  190.993017\_13.118464 & ngc4654 & 190.99302 & 13.11846 & 2562.0 & 2324.64 & 20.52 & 0.05 & 20.84 & 0.05 & 21.88 & 0.05 & 21.87 & 0.05 & 21.42 & 0.07 & 7.0 & 25.0 & 13363.6 & 31681.35 & 0.13 & 0.12 & -1.25 & 3.0\\
  190.991433\_13.11943 & ngc4654 & 190.99143 & 13.11943 & 2702.65 & 2412.24 & 21.33 & 0.05 & 21.37 & 0.05 & 22.22 & 0.04 & 22.14 & 0.04 & 21.62 & 0.04 & 4.0 & 2.0 & 24430.45 & 7949.29 & 0.47 & 0.14 & -1.4 & 3.0\\
  190.994316\_13.138858 & ngc4654 & 190.99432 & 13.13886 & 2447.18 & 4177.95 & 20.19 & 0.02 & 20.5 & 0.02 & 21.93 & 0.02 & 21.92 & 0.02 & 21.88 & 0.04 & 1.0 & 3.0 & 37892.09 & 27556.1 & 0.26 & 0.12 & -1.51 & 3.0\\
  190.970888\_13.13849 & ngc4654 & 190.97089 & 13.13849 & 4520.5 & 4144.99 & 20.29 & 0.04 & 20.57 & 0.03 & 21.86 & 0.04 & 21.6 & 0.03 & 20.96 & 0.03 & 19.0 & 2.0 & 43490.08 & 8921.88 & 0.05 & 0.03 & -1.09 & 3.0\\
  190.994703\_13.139378 & ngc4654 & 190.9947 & 13.13938 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & -0.74 & 3.0\\
  191.944488\_13.781038 & ngc4689 & 191.94449 & 13.78104 & 3422.27 & 5362.78 & 23.37 & 0.16 & 22.71 & 0.08 & 22.77 & 0.03 & 22.13 & 0.01 & 21.08 & 0.01 & 147.0 & 35.0 & 132700.27 & 4325.93 & 0.46 & 0.06 & -1.82 & 1.0\\
  191.94729\_13.75244 & ngc4689 & 191.94729 & 13.75244 & 3174.65 & 2764.08 & 19.39 & 0.01 & 19.87 & 0.01 & 21.11 & 0.01 & 21.17 & 0.01 & 20.62 & 0.01 & 8.0 & 0.0 & 10631.03 & 837.44 & 0.01 & 0.02 & -1.56 & 1.0\\
  191.935382\_13.767092 & ngc4689 & 191.93538 & 13.76709 & 4225.79 & 4095.59 & 25.12 & 0.83 & 23.26 & 0.14 & 22.8 & 0.03 & 21.92 & 0.02 & 20.6 & 0.01 & 8925.0 & 4582.0 & 1054202.94 & 422416.83 & 0.0 & 0.02 & -1.85 & 1.0\\
  191.936075\_13.765091 & ngc4689 & 191.93608 & 13.76509 & 4164.6 & 3913.79 & 23.29 & 0.21 & 22.41 & 0.07 & 22.47 & 0.03 & 21.94 & 0.02 & 20.88 & 0.02 & 169.0 & 41.0 & 164965.41 & 16731.85 & 0.43 & 0.08 & -1.82 & 1.0\\
  191.923348\_13.759875 & ngc4689 & 191.92335 & 13.75988 & 5287.79 & 3439.88 & 24.9 & 0.66 & 23.72 & 0.2 & 23.32 & 0.04 & 22.24 & 0.02 & 20.89 & 0.01 & 10308.0 & 9418.0 & 1006034.78 & 660105.18 & 0.06 & 0.36 & -1.57 & 1.0\\
  191.942035\_13.751533 & ngc4689 & 191.94204 & 13.75153 & 3638.84 & 2681.36 & 20.07 & 0.01 & 20.47 & 0.01 & 21.92 & 0.01 & 21.94 & 0.01 & 21.62 & 0.02 & 1.0 & 1.0 & 20271.92 & 6250.92 & 0.28 & 0.04 & -1.74 & 1.0\\
  191.936892\_13.773706 & ngc4689 & 191.93689 & 13.77371 & 4092.52 & 4696.58 & 23.01 & 0.11 & 22.0 & 0.04 & 21.87 & 0.01 & 21.15 & 0.01 & 20.02 & 0.01 & 1276.0 & 320.0 & 455838.42 & 14792.16 & 0.05 & 0.09 & -1.84 & 1.0\\
  191.935898\_13.748252 & ngc4689 & 191.9359 & 13.74825 & 4180.32 & 2383.6 & 21.69 & 0.04 & 21.8 & 0.04 & 22.04 & 0.02 & 21.96 & 0.01 & 21.44 & 0.02 & 182.0 & 55.0 & 48236.2 & 3115.18 & 0.0 & 0.06 & -1.68 & 1.0\\
  191.949913\_13.755348 & ngc4689 & 191.94991 & 13.75535 & 2943.22 & 3028.4 & 19.22 & 0.01 & 19.63 & 0.01 & 20.83 & 0.01 & 20.93 & 0.01 & 20.45 & 0.01 & 8.0 & 1.0 & 13002.81 & 1497.65 & 0.01 & 0.02 & -1.58 & 1.0\\
  191.930271\_13.754802 & ngc4689 & 191.93027 & 13.7548 & 4676.74 & 2978.78 & 24.04 & 0.3 & 23.55 & 0.17 & 23.11 & 0.03 & 22.32 & 0.02 & 20.95 & 0.01 & 196.0 & 471.0 & 255335.98 & 1299.83 & 0.67 & 0.28 & -1.74 & 1.0\\
  191.927346\_13.773213 & ngc4689 & 191.92735 & 13.77321 & 4934.85 & 4651.87 & 19.4 & 0.01 & 19.61 & 0.01 & 20.76 & 0.01 & 20.75 & 0.01 & 20.6 & 0.01 & 4.0 & 1.0 & 21223.75 & 3962.36 & 0.27 & 0.08 & -1.48 & 2.0\\
  191.930631\_13.772852 & ngc4689 & 191.93063 & 13.77285 & 4644.74 & 4618.21 & 20.67 & 0.02 & 20.77 & 0.02 & 22.05 & 0.02 & 21.81 & 0.02 & 21.15 & 0.02 & 8.0 & 0.0 & 8896.08 & 1063.12 & 0.17 & 0.03 & -1.69 & 2.0\\
  191.944772\_13.773688 & ngc4689 & 191.94477 & 13.77369 & 3397.06 & 4695.0 & 20.22 & 0.01 & 20.64 & 0.02 & 22.01 & 0.02 & 21.98 & 0.01 & 21.59 & 0.02 & 8.0 & 0.0 & 4645.71 & 176.24 & 0.0 & 0.01 & -1.77 & 2.0\\
  191.9364\_13.752839 & ngc4689 & 191.9364 & 13.75284 & 4135.9 & 2800.29 & 21.02 & 0.03 & 20.99 & 0.03 & 22.13 & 0.02 & 21.96 & 0.02 & 21.34 & 0.02 & 1.0 & 2.0 & 46266.94 & 20063.28 & 0.56 & 0.05 & -1.71 & 2.0\\
  191.94327\_13.765516 & ngc4689 & 191.94327 & 13.76552 & 3529.81 & 3952.08 & 17.68 & 0.01 & 18.15 & 0.01 & 19.73 & 0.01 & 19.85 & 0.01 & 19.76 & 0.02 & 1.0 & 2.0 & 94412.52 & 39076.48 & 0.16 & 0.04 & -1.59 & 2.0\\
  191.935415\_13.755163 & ngc4689 & 191.93541 & 13.75516 & 4223.2 & 3012.43 & 20.02 & 0.01 & 20.59 & 0.02 & 22.16 & 0.02 & 22.32 & 0.02 & 22.45 & 0.05 & 1.0 & 0.0 & 7684.45 & 1180.9 & 0.1 & 0.04 & -1.29 & 2.0\\
  191.931444\_13.757587 & ngc4689 & 191.93144 & 13.75759 & 4573.24 & 3231.76 & 20.86 & 0.03 & 20.99 & 0.03 & 21.43 & 0.01 & 21.21 & 0.01 & 20.77 & 0.01 & 136.0 & 33.0 & 79790.31 & 8272.34 & 0.02 & 0.02 & -1.79 & 2.0\\
  191.935114\_13.752908 & ngc4689 & 191.93511 & 13.75291 & 4249.3 & 2806.83 & 20.79 & 0.02 & 21.02 & 0.02 & 22.34 & 0.02 & 22.39 & 0.02 & 22.28 & 0.04 & 3.0 & 1.0 & 8763.8 & 4528.22 & 0.29 & 0.07 & -1.73 & 2.0\\
  191.954343\_13.764341 & ngc4689 & 191.95434 & 13.76434 & 2553.06 & 3845.52 & 20.42 & 0.02 & 20.84 & 0.02 & 22.35 & 0.02 & 22.4 & 0.02 & 22.17 & 0.03 & 1.0 & 0.0 & 11225.82 & 1866.4 & 0.23 & 0.04 & -1.66 & 2.0\\
  191.9288\_13.761272 & ngc4689 & 191.9288 & 13.76127 & 4806.64 & 3566.95 & 18.46 & 0.01 & 18.92 & 0.01 & 20.49 & 0.01 & 20.54 & 0.01 & 20.53 & 0.02 & 1.0 & 2.0 & 49210.41 & 14131.13 & 0.17 & 0.01 & -1.79 & 2.0\\
  191.933551\_13.768611 & ngc4689 & 191.93355 & 13.76861 & 4387.370881200778 & 4233.492430889669 & 20.65 & 0.02 & 20.98 & 0.03 & 22.29 & 0.03 & 22.32 & 0.03 & 22.36 & 0.06 & 4.0 & 3.0 & 3365.06 & 10518.03 & 0.15 & 0.15 & -0.87 & 3.0\\
  191.935901\_13.776565 & ngc4689 & 191.9359 & 13.77656 & 4179.97 & 4955.7 & 21.63 & 0.05 & 22.11 & 0.06 & 23.07 & 0.04 & 23.12 & 0.04 & 22.83 & 0.06 & 6.0 & 1.0 & 1508.5 & 433.9 & 0.1 & 0.08 & -1.24 & 3.0\\
  191.931179\_13.757855 & ngc4689 & 191.93118 & 13.75786 & 4596.76 & 3255.68 & 21.52 & 0.05 & 21.66 & 0.04 & 22.99 & 0.04 & 22.93 & 0.05 & 22.8 & 0.11 & 3.0 & 1.0 & 6032.19 & 186.05 & 0.34 & 0.03 & -0.62 & 3.0\\
  191.947669\_13.77423 & ngc4689 & 191.94767 & 13.77423 & 3141.44 & 4743.7 & 21.19 & 0.07 & 21.68 & 0.06 & 23.06 & 0.07 & 23.0 & 0.07 & 21.57 & 0.03 & 10.0 & 1.0 & 5504.31 & 28.45 & 0.13 & 0.05 & -1.54 & 3.0\\
  191.946532\_13.772254 & ngc4689 & 191.94653 & 13.77225 & 3240.89 & 4564.85 & 22.88 & 0.14 & 23.16 & 0.15 & 24.37 & 0.16 & 24.4 & 0.19 & 24.32 & 0.33 & 4.0 & 3.0 & 612.27 & 26.12 & 0.21 & 0.08 & -0.62 & 3.0\\
  191.950983\_13.760106 & ngc4689 & 191.95098 & 13.76011 & 2848.95 & 3460.66 & 21.3 & 0.04 & 21.88 & 0.05 & 23.36 & 0.05 & 23.59 & 0.05 & 23.94 & 0.16 & 3.0 & 2.0 & 1383.19 & 354.9 & 0.06 & 0.03 & -1.2 & 3.0\\
  191.954292\_13.760951 & ngc4689 & 191.95429 & 13.76095 & 2556.89 & 3537.4 & 21.07 & 0.07 & 21.26 & 0.06 & 22.07 & 0.04 & 22.0 & 0.04 & 21.73 & 0.04 & 5.0 & 1.0 & 7302.47 & 1991.72 & 0.3 & 0.09 & -1.61 & 3.0\\
  191.934574\_13.773127 & ngc4689 & 191.93457 & 13.77313 & 4296.97 & 4644.04 & 20.71 & 0.02 & 21.21 & 0.03 & 22.51 & 0.02 & 22.59 & 0.03 & 22.61 & 0.05 & 4.0 & 1.0 & 2381.54 & 3847.53 & 0.11 & 0.13 & -0.91 & 3.0\\
  194.190374\_21.695519 & ngc4826 & 194.19037 & 21.69552 & 3108.47 & 4889.53 & 23.88 & 0.3 & 22.5 & 0.07 & 22.13 & 0.02 & 21.4 & 0.01 & 20.15 & 0.01 & 1028.0 & 451.0 & 44058.25 & 2977.8 & 0.23 & 0.17 & -1.8 & 1.0\\
  194.170181\_21.694304 & ngc4826 & 194.17018 & 21.6943 & 4813.18 & 4779.13 & 23.29 & 0.19 & 22.12 & 0.06 & 22.05 & 0.02 & 21.52 & 0.02 & 20.76 & 0.02 & 890.0 & 223.0 & 17412.43 & 1584.54 & 0.0 & 0.05 & -1.68 & 1.0\\
  194.161467\_21.693118 & ngc4826 & 194.16147 & 21.69312 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & -1.5 & 1.0\\
  194.173786\_21.684177 & ngc4826 & 194.17379 & 21.68418 & 4509.03 & 3859.1 & 20.45 & 0.02 & 20.34 & 0.02 & 20.85 & 0.01 & 20.7 & 0.01 & 20.03 & 0.02 & 110.0 & 37.0 & 14788.62 & 238.52 & 0.12 & 0.05 & -1.74 & 1.0\\
  194.162992\_21.685389 & ngc4826 & 194.16299 & 21.68539 & 5420.15 & 3969.43 & 21.88 & 0.06 & 21.22 & 0.03 & 21.21 & 0.01 & 20.62 & 0.01 & 19.52 & 0.01 & 169.0 & 42.0 & 53902.22 & 3833.77 & 0.47 & 0.08 & -1.72 & 1.0\\
  194.160047\_21.685459 & ngc4826 & 194.16005 & 21.68546 & 5668.81 & 3975.62 & 22.18 & 0.07 & 21.58 & 0.04 & 21.7 & 0.02 & 21.13 & 0.01 & 20.08 & 0.01 & 118.0 & 51.0 & 28317.42 & 2989.51 & 0.48 & 0.04 & -1.71 & 1.0\\
  194.170105\_21.683517 & ngc4826 & 194.1701 & 21.68352 & 4819.55 & 3799.14 & 18.88 & 0.01 & 19.09 & 0.01 & 20.36 & 0.01 & 20.43 & 0.01 & 20.34 & 0.02 & 4.0 & 3.0 & 2027.98 & 5947.66 & 0.2 & 0.14 & -1.84 & 1.0\\
  194.18784\_21.671258 & ngc4826 & 194.18784 & 21.67126 & 3322.27 & 2685.14 & 20.78 & 0.03 & 20.25 & 0.01 & 20.42 & 0.01 & 19.85 & 0.01 & 18.76 & 0.01 & 5.0 & 83.0 & 28741.84 & 62031.48 & 0.91 & 0.38 & -1.72 & 1.0\\
  194.179797\_21.678429 & ngc4826 & 194.1798 & 21.67843 & 4001.31 & 3336.71 & 22.35 & 0.09 & 21.43 & 0.04 & 21.55 & 0.02 & 20.96 & 0.01 & 19.84 & 0.02 & 169.0 & 11.0 & 39680.63 & 4727.53 & 0.47 & 0.05 & -1.63 & 1.0\\
  194.18759\_21.670516 & ngc4826 & 194.18759 & 21.67052 & 3343.28 & 2617.92 & 21.11 & 0.03 & 21.11 & 0.03 & 21.42 & 0.01 & 21.3 & 0.01 & 20.42 & 0.02 & 95.0 & 32.0 & 10284.34 & 1515.75 & 0.2 & 0.02 & -1.62 & 1.0\\
  194.183377\_21.665994 & ngc4826 & 194.18338 & 21.66599 & 3699.1 & 2207.07 & 19.6 & 0.01 & 19.12 & 0.01 & 19.23 & 0.0 & 18.64 & 0.0 & 17.55 & 0.0 & 110.0 & 48.0 & 289842.09 & 10009.5 & 0.5 & 0.08 & -1.69 & 1.0\\
  194.178782\_21.690269 & ngc4826 & 194.17878 & 21.69027 & 4087.13 & 4413.06 & 21.0 & 0.03 & 20.29 & 0.02 & 20.32 & 0.01 & 19.7 & 0.01 & 18.55 & 0.01 & 158.0 & 38.0 & 132094.2 & 19941.33 & 0.5 & 0.01 & -1.69 & 2.0\\
  194.16901\_21.684917 & ngc4826 & 194.16901 & 21.68492 & 4912.27 & 3926.22 & 19.26 & 0.01 & 18.98 & 0.01 & 19.94 & 0.01 & 19.85 & 0.01 & 19.53 & 0.01 & 5.0 & 1.0 & 5680.88 & 2114.85 & 0.37 & 0.11 & -1.87 & 2.0\\
  194.181926\_21.677512 & ngc4826 & 194.18193 & 21.67751 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & -1.44 & 2.0\\
  194.170152\_21.68923 & ngc4826 & 194.17015 & 21.68923 & 4815.82 & 4318.11 & 17.5 & 0.01 & 18.05 & 0.01 & 19.59 & 0.01 & 19.75 & 0.01 & 19.6 & 0.01 & 1.0 & 2.0 & 9208.26 & 2895.59 & 0.16 & 0.0 & -1.76 & 2.0\\
  194.170648\_21.688271 & ngc4826 & 194.17065 & 21.68827 & 4773.92 & 4230.79 & 17.03 & 0.01 & 17.5 & 0.01 & 19.02 & 0.01 & 19.14 & 0.01 & 19.17 & 0.02 & 1.0 & 2.0 & 15084.79 & 4328.75 & 0.16 & 0.01 & -1.28 & 2.0\\
  194.169814\_21.683716 & ngc4826 & 194.16981 & 21.68372 & 4844.35 & 3817.27 & 19.05 & 0.01 & 19.5 & 0.01 & 21.01 & 0.02 & 21.12 & 0.02 & 21.38 & 0.06 & 3.0 & 2.0 & 1311.85 & 504.63 & 0.11 & 0.01 & -1.52 & 2.0\\
  194.178422\_21.681486 & ngc4826 & 194.17842 & 21.68149 & 4117.6 & 3614.48 & 17.72 & 0.01 & 17.26 & 0.01 & 18.25 & 0.0 & 18.2 & 0.0 & 17.75 & 0.01 & 4.0 & 0.0 & 40530.72 & 4790.95 & 0.51 & 0.03 & -1.95 & 2.0\\
  194.175025\_21.685545 & ngc4826 & 194.17502 & 21.68554 & 4404.41 & 3983.36 & 20.81 & 0.03 & 20.78 & 0.02 & 21.25 & 0.02 & 21.0 & 0.02 & 20.17 & 0.02 & 76.0 & 19.0 & 12675.08 & 2483.2 & 0.23 & 0.0 & -1.58 & 2.0\\
  194.176872\_21.682819 & ngc4826 & 194.17687 & 21.68282 & 4248.77 & 3735.79 & 17.85 & 0.01 & 18.2 & 0.01 & 19.64 & 0.01 & 19.71 & 0.01 & 19.54 & 0.02 & 1.0 & 1.0 & 12117.12 & 3391.84 & 0.25 & 0.03 & -1.8 & 2.0\\
  194.173346\_21.68082 & ngc4826 & 194.17335 & 21.68082 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & -1.53 & 2.0\\
  194.170007\_21.689438 & ngc4826 & 194.17001 & 21.68944 & 4828.59 & 4336.96 & 19.84 & 0.05 & 20.35 & 0.05 & 21.77 & 0.07 & 21.8 & 0.06 & 21.1 & 0.05 & 9.0 & 1.0 & 688.16 & 85.73 & 0.0 & 0.03 & -1.17 & 3.0\\
  194.170527\_21.689804 & ngc4826 & 194.17053 & 21.6898 & 4784.3 & 4369.83 & 19.89 & 0.02 & 20.43 & 0.03 & 21.78 & 0.03 & 21.84 & 0.04 & 21.32 & 0.05 & 8.0 & 0.0 & 499.8 & 19.52 & 0.0 & 0.01 & -1.14 & 3.0\\
  194.178494\_21.688706 & ngc4826 & 194.17849 & 21.68871 & 4112.05 & 4271.15 & 18.97 & 0.02 & 19.45 & 0.03 & 21.11 & 0.03 & 21.25 & 0.03 & 21.08 & 0.05 & 1.0 & 2.0 & 2081.19 & 590.77 & 0.13 & 0.01 & -0.76 & 3.0\\
  194.180283\_21.687905 & ngc4826 & 194.18028 & 21.6879 & 3959.65 & 4197.65 & 19.94 & 0.02 & 19.83 & 0.02 & 20.78 & 0.01 & 20.52 & 0.02 & 19.91 & 0.02 & 3.0 & 1.0 & 11858.27 & 6120.81 & 0.63 & 0.07 & -0.84 & 3.0\\
  194.185221\_21.686866 & ngc4826 & 194.18522 & 21.68687 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & -0.87 & 3.0\\
  194.177258\_21.686718 & ngc4826 & 194.17726 & 21.68672 & 4215.94 & 4089.93 & 20.15 & 0.03 & 20.08 & 0.03 & 20.96 & 0.02 & 20.8 & 0.03 & 20.38 & 0.07 & 4.0 & 2.0 & 3436.11 & 6326.31 & 0.49 & 0.11 & -1.58 & 3.0\\
  194.176258\_21.684588 & ngc4826 & 194.17626 & 21.68459 & 4300.4 & 3896.18 & 18.88 & 0.01 & 19.23 & 0.01 & 20.61 & 0.01 & 20.68 & 0.02 & 20.86 & 0.06 & 4.0 & 1.0 & 1115.9 & 1696.3 & 0.1 & 0.12 & -0.95 & 3.0\\
  194.173144\_21.687519 & ngc4826 & 194.17314 & 21.68752 & 4563.16 & 4162.67 & 20.25 & 0.1 & 20.5 & 0.08 & 20.75 & 0.02 & 20.16 & 0.01 & 19.37 & 0.01 & 88.0 & 22.0 & 34456.94 & 301.04 & 0.33 & 0.05 & -1.24 & 3.0\\
  194.178479\_21.688686 & ngc4826 & 194.17848 & 21.68869 & 4113.47 & 4268.16 & 19.12 & 0.02 & 19.6 & 0.02 & 21.29 & 0.02 & 21.44 & 0.03 & 21.66 & 0.08 & 1.0 & 0.0 & 1340.53 & 213.37 & 0.07 & 0.04 & -0.79 & 3.0\\
  194.180312\_21.687926 & ngc4826 & 194.18031 & 21.68793 & 3957.94 & 4199.57 & 20.25 & 0.02 & 20.02 & 0.02 & 20.85 & 0.01 & 20.5 & 0.01 & 19.7 & 0.02 & 2.0 & 2.0 & 21625.27 & 13428.83 & 0.76 & 0.09 & -1.24 & 3.0\\
  194.17796\_21.68389 & ngc4826 & 194.17796 & 21.68389 & 4156.55 & 3832.81 & 21.05 & 0.11 & 21.04 & 0.1 & 21.38 & 0.05 & 21.55 & 0.07 & 20.81 & 0.08 & 136.0 & 33.0 & 5925.85 & 1521.09 & 0.01 & 0.02 & -0.88 & 3.0\\
  204.399643\_8.904539 & ngc5248 & 204.39964 & 8.90454 & 2350.89 & 5781.02 & 24.02 & 0.3 & 23.59 & 0.15 & 23.54 & 0.04 & 22.96 & 0.02 & 21.78 & 0.02 & 136.0 & 131.0 & 69541.35 & 47658.87 & 0.5 & 0.46 & -1.46 & 1.0\\
  204.401661\_8.888672 & ngc5248 & 204.40166 & 8.88867 & 2169.48 & 4338.79 & 27.12 & 5.48 & 24.91 & 0.56 & 24.09 & 0.08 & 22.84 & 0.02 & 21.21 & 0.01 & 13750.0 & 13173.0 & 1244654.27 & 868780.61 & 0.23 & 0.53 & -1.61 & 1.0\\
  204.38244\_8.897404 & ngc5248 & 204.38244 & 8.8974 & 3895.21 & 5132.83 & 22.98 & 0.12 & 22.91 & 0.09 & 22.61 & 0.02 & 22.37 & 0.02 & 21.69 & 0.02 & 349.0 & 106.0 & 55380.21 & 491.37 & 0.06 & 0.09 & -1.63 & 1.0\\
  204.392309\_8.894962 & ngc5248 & 204.39231 & 8.89496 & 3009.22 & 4910.87 & 22.86 & 0.11 & 21.99 & 0.04 & 22.11 & 0.02 & 21.51 & 0.01 & 20.38 & 0.01 & 147.0 & 49.0 & 264325.8 & 5073.27 & 0.49 & 0.07 & -1.68 & 1.0\\
  204.38224\_8.90365 & ngc5248 & 204.38224 & 8.90365 & 3913.09 & 5700.3 & 23.76 & 0.23 & 22.61 & 0.07 & 22.45 & 0.02 & 21.7 & 0.01 & 20.42 & 0.01 & 2271.0 & 995.0 & 481876.81 & 58263.93 & 0.04 & 0.15 & -1.73 & 1.0\\
  204.385929\_8.887824 & ngc5248 & 204.38593 & 8.88782 & 3581.98 & 4262.16 &  & -1.56 & 23.55 & 0.19 & 23.07 & 0.04 & 22.33 & 0.02 & 21.18 & 0.02 & 828.0 & 874.0 & 195218.82 & 63962.48 & 0.26 & 0.12 & -1.79 & 1.0\\
  204.386761\_8.88979 & ngc5248 & 204.38676 & 8.88979 & 3507.53 & 4440.83 & 23.69 & 0.24 & 23.36 & 0.14 & 23.26 & 0.04 & 22.66 & 0.03 & 21.52 & 0.02 & 147.0 & 71.0 & 91042.05 & 11534.92 & 0.49 & 0.08 & -1.69 & 1.0\\
  204.379831\_8.886564 & ngc5248 & 204.37983 & 8.88656 & 4129.34 & 4147.78 & 23.79 & 0.29 & 22.78 & 0.09 & 22.77 & 0.03 & 22.26 & 0.02 & 21.12 & 0.02 & 182.0 & 142.0 & 143759.44 & 12162.77 & 0.46 & 0.14 & -1.79 & 1.0\\
  204.365527\_8.87294 & ngc5248 & 204.36553 & 8.87294 & 5413.64 & 2910.15 & 25.38 & 1.0 & 25.29 & 0.81 & 24.45 & 0.1 & 23.27 & 0.03 & 21.76 & 0.02 & 13750.0 & 956.0 & 643812.9 & 148053.04 & 0.14 & 0.08 & -1.39 & 1.0\\
  204.371613\_8.860308 & ngc5248 & 204.37161 & 8.86031 & 4867.08 & 1762.08 & 24.16 & 0.34 & 23.64 & 0.17 & 23.67 & 0.05 & 23.02 & 0.02 & 21.83 & 0.02 & 110.0 & 151.0 & 69897.69 & 10380.54 & 0.56 & 0.11 & -1.57 & 1.0\\
  204.374382\_8.900841 & ngc5248 & 204.37438 & 8.90084 & 4618.59 & 5445.13 & 19.05 & 0.01 & 19.34 & 0.01 & 20.45 & 0.01 & 20.5 & 0.01 & 20.02 & 0.01 & 7.0 & 1.0 & 20444.76 & 107.86 & 0.1 & 0.04 & -1.75 & 2.0\\
  204.368245\_8.896542 & ngc5248 & 204.36824 & 8.89654 & 5169.27 & 5054.47 & 18.49 & 0.01 & 18.82 & 0.01 & 19.98 & 0.01 & 19.89 & 0.01 & 19.22 & 0.01 & 8.0 & 5.0 & 46425.86 & 10144.52 & 0.12 & 0.11 & -1.64 & 2.0\\
  204.383228\_8.892481 & ngc5248 & 204.38323 & 8.89248 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & -1.35 & 2.0\\
  204.38348\_8.89155 & ngc5248 & 204.38348 & 8.89155 & 3801.77 & 4600.76 & 18.55 & 0.01 & 18.74 & 0.01 & 19.86 & 0.01 & 19.82 & 0.01 & 19.16 & 0.01 & 8.0 & 26.0 & 52490.57 & 103778.58 & 0.14 & 0.11 & -1.78 & 2.0\\
  204.368528\_8.887676 & ngc5248 & 204.36853 & 8.88768 & 5144.06 & 4248.95 & 21.24 & 0.03 & 21.08 & 0.03 & 21.13 & 0.01 & 21.01 & 0.01 & 20.39 & 0.01 & 261.0 & 41.0 & 145926.72 & 8599.89 & 0.02 & 0.02 & -1.68 & 2.0\\
  204.3966\_8.870584 & ngc5248 & 204.3966 & 8.87058 & 2624.07 & 2695.36 & 18.56 & 0.01 & 18.87 & 0.01 & 20.37 & 0.01 & 20.36 & 0.02 & 20.17 & 0.02 & 1.0 & 2.0 & 79819.22 & 33012.65 & 0.27 & 0.04 & -1.6 & 2.0\\
  204.375325\_8.875519 & ngc5248 & 204.37532 & 8.87552 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & -1.34 & 2.0\\
  204.397374\_8.873061 & ngc5248 & 204.39737 & 8.87306 & 2554.02 & 2920.71 & 19.85 & 0.02 & 20.34 & 0.02 & 21.73 & 0.02 & 21.83 & 0.02 & 21.79 & 0.03 & 1.0 & 1.0 & 16823.27 & 1489.66 & 0.21 & 0.03 & -1.53 & 2.0\\
  204.389673\_8.889171 & ngc5248 & 204.38967 & 8.88917 & 3245.89 & 4384.61 & 19.24 & 0.01 & 19.32 & 0.01 & 20.26 & 0.01 & 20.14 & 0.01 & 19.33 & 0.01 & 8.0 & 22.0 & 56121.9 & 73804.22 & 0.26 & 0.15 & -1.8 & 2.0\\
  204.396675\_8.870809 & ngc5248 & 204.39668 & 8.87081 & 2617.64 & 2715.9 & 18.31 & 0.02 & 18.82 & 0.02 & 20.25 & 0.02 & 20.3 & 0.02 & 20.14 & 0.03 & 1.0 & 0.0 & 74952.42 & 11198.94 & 0.23 & 0.04 & -1.08 & 3.0\\
  204.373955\_8.900769 & ngc5248 & 204.37396 & 8.90077 & 4657.04 & 5438.4 & 20.63 & 0.04 & 20.93 & 0.04 & 22.04 & 0.05 & 22.06 & 0.05 & 21.7 & 0.07 & 6.0 & 3.0 & 4325.76 & 14324.82 & 0.12 & 0.3 & -0.67 & 3.0\\
  204.383312\_8.89207 & ngc5248 & 204.38331 & 8.89207 & 3816.66 & 4648.04 & 19.63 & 0.03 & 20.09 & 0.04 & 21.59 & 0.04 & 21.69 & 0.04 & 21.75 & 0.06 & 1.0 & 3.0 & 16698.23 & 11764.58 & 0.17 & 0.1 & -1.44 & 3.0\\
  204.402338\_8.87143 & ngc5248 & 204.40234 & 8.87143 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & -1.9 & 3.0\\
  204.383409\_8.891398 & ngc5248 & 204.38341 & 8.8914 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & -0.91 & 3.0\\
  204.382838\_8.891625 & ngc5248 & 204.38284 & 8.89162 & 3859.38 & 4607.46 & 20.87 & 0.08 & 21.01 & 0.06 & 22.09 & 0.05 & 22.08 & 0.05 & 21.51 & 0.03 & 7.0 & 0.0 & 5919.47 & 803.08 & 0.17 & 0.04 & -1.21 & 3.0\\
  204.38095\_8.895612 & ngc5248 & 204.38095 & 8.89561 & 4028.58 & 4970.47 & 19.78 & 0.01 & 19.95 & 0.02 & 21.28 & 0.01 & 21.27 & 0.01 & 20.96 & 0.02 & 1.0 & 2.0 & 47647.37 & 20766.6 & 0.37 & 0.05 & -1.14 & 3.0\\
  204.397478\_8.871182 & ngc5248 & 204.39748 & 8.87118 & 2545.18 & 2749.92 & 19.55 & 0.03 & 19.93 & 0.03 & 21.38 & 0.03 & 21.42 & 0.03 & 21.29 & 0.06 & 1.0 & 2.0 & 27048.38 & 6893.82 & 0.24 & 0.02 & -0.64 & 3.0\\
\bottomrule
\end{tabularx}
\end{sidewaystable}
